SAUC: Sparsity-Aware Uncertainty Calibration for Spatiotemporal Prediction with Graph Neural Networks

Quantifying uncertainty is crucial for robust and reliable predictions. However, existing spatiotemporal deep learning mostly focuses on deterministic prediction, overlooking the inherent uncertainty in such prediction. Particularly, highly-granular spatiotemporal datasets are often sparse, posing extra challenges in prediction and uncertainty quantification. To address these issues, this paper introduces a novel post-hoc Sparsity-awar Uncertainty Calibration (SAUC) framework, which calibrates uncertainty in both zero and non-zero values. To develop SAUC, we firstly modify the state-of-the-art deterministic spatiotemporal Graph Neural Networks (ST-GNNs) to probabilistic ones in the pre-calibration phase. Then we calibrate the probabilistic ST-GNNs for zero and non-zero values using quantile approaches.Through extensive experiments, we demonstrate that SAUC can effectively fit the variance of sparse data and generalize across two real-world spatiotemporal datasets at various granularities. Specifically, our empirical experiments show a 20\% reduction in calibration errors in zero entries on the sparse traffic accident and urban crime prediction. Overall, this work demonstrates the theoretical and empirical values of the SAUC framework, thus bridging a significant gap between uncertainty quantification and spatiotemporal prediction.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> backup_KDD_sections/1.Introduction.tex <==
\section{Introduction}

Spatiotemporal Graph Neural Networks (GNNs) have been instrumental in leveraging spatiotemporal data for various applications, from weather forecasting to urban planning \citep{wu2021inductive, zhao2022multi,gao2023spatiotemporal}. However, most of the models are narrowly focused on deterministic predictions, which overlooks the inherent uncertainties associated with the spatiotemporal phenomena. For various safety-related tasks, such as traffic accidents and urban crime prediction, it is crucial to quantify their uncertainty, thus proactively preventing such phenomena from happening. Despite its importance, uncertainty quantification (UQ) remains relatively understudied in the spatiotemporal context, which can lead to erroneous predictions with severe social consequences \citep{chung2021beyond,abdo2017uncertainty,rudin2019stop}.

Recent research has addressed UQ in spatiotemporal modeling \citep{wang2023uncertainty,zhuang2022uncertainty,huang_uncertainty_2023}, but often fails to account for the sparsity and asymmetrical distribution present in detailed spatiotemporal data. This sparsity, marked by an abundance of zeros, becomes essential when working with high-resolution data. Additionally, the need for granular forecasting in event precaution often leads to more diluted inputs, making sparsity unavoidable. Thus, effectively managing aleatoric (data) uncertainty is crucial in these forecasting tasks.

Prior spatiotemporal GNNs with basic UQ functionalities typically model data using Negative Binomial (NB) or Gaussian distributions for regression tasks, focusing on learning these distributions' parameters for spatiotemporal predictions \citep{jiang2023uncertainty,zhuang2022uncertainty,wang2023uncertainty}. A key limitation is their inadequate evaluation of UQ reliability using robust calibration metrics. Research by \citep{zhuang2022uncertainty,wu2021quantifying,jiang2023uncertainty,gao2023spatiotemporal} often emphasizes high accuracy and narrow prediction intervals as indicators of effective UQ. This approach overlooks the crucial relationship between data variance and prediction intervals (PI), which is vital for addressing aleatoric uncertainty. As highlighted by \citep{kuleshov2018accurate}, most deep learning models are not fully calibrated for high UQ quality, leaving a significant research gap to be filled.

This paper introduces a sparsity-aware uncertainty calibration (SAUC) method, calibrating model outputs to align with true data distributions, which can be adapted to any spatiotemporal GNN model. Inspired by the zero-inflated model, we partition zero and non-zero predictions and apply separate Quantile Regression (QR) models to ensure the discrepancy of prediction and true values lie within the PIs. This post-hoc approach, unlike uncertainty-aware spatiotemporal prediction models \citep{rahman_uncertainty-aware_2023}, offers flexibility in applying it to existing models without necessitating architectural changes or full model retraining. Consistent with prior studies on regression task calibration, we formulate a modified calibration metric tailored for PI-based calibration within asymmetric distributions. To investigate our model's generalizability, we adapt three prevalent spatiotemporal GNN models with negative binomial distributions to accommodate sparse settings without compromising prediction accuracy. Tested on two real-world spatiotemporal datasets with different levels of sparsity, our SAUC demonstrates promising calibration results, thus assisting in reliable decision-making and risk assessment.
The main contributions of this paper are threefold:
\begin{itemize}
    \item We have developed a novel post-hoc uncertainty calibration method tailored for predicting sparse spatiotemporal data. This approach is designed to be compatible with current GNN models and is suitable for any probabilistic outputs.
    \item We focus on calibrating asymmetric distributions, like the NB, using quantile regression. This approach deviates from conventional mean-variance UQ methods. Additionally, we have developed new calibration metrics based on prediction interval width.
    \item We conduct experiments on real-world datasets with different temporal resolutions to demonstrate promising calibration results of our SAUC, especially for zero values. We observe a roughly \textbf{20\% reduction} in calibration errors relative to leading baseline models, underscoring its efficacy for safety-critical decision-making.
\end{itemize}


==> backup_KDD_sections/2.RelatedWork.tex <==
\section{Related Work}
% \subsection{DL in Spatiotemporal Prediction}
% \redfont{Existing work do not consider UQ first }

\subsection{Spatiotemporal Prediction}

% \subsection{UQ in Spatiotemporal Deep Learning}
% Spatiotemporal prediction leveraging deep learning and Graph Neural Networks (GNNs) has emerged as a powerful tool in machine learning, providing invaluable insights for diverse applications, including traffic forecasting, climate modeling, and urban planning. However, there's a significant research gap regarding Uncertainty Quantification (UQ) in these models. The lack of focus on UQ leads to overlooked uncertainties in predictions, compromising their reliability.

% UQ in spatiotemporal prediction plays a crucial role in measuring the confidence and reliability of the prediction results. Two principal methodologies have been employed for this purpose, namely, the Bayesian and Frequentist approaches \citep{wang2023uncertainty, zhuang2022uncertainty,zhao2022multi}. The Bayesian paradigm, grounded in parameter inference techniques such as Laplace approximation, Markov Chain Monte Carlo (MCMC), and Variational Inference (VI), offers critical insights. However, it is often hampered by computational complexities and inaccuracies arising from approximation \citep{wu2021bayesian,qian2022uncertainty,wu2021quantifying,gawlikowski2021survey}.

% On the contrary, the Frequentist approach leverages Mean-Variance Estimation (MVE), leading to computational efficiency and flexibility in model construction \citep{wang2023uncertainty}. This approach encompasses both parametric and non-parametric methods, with the former incorporating probabilistic layers for UQ, and the latter primarily focusing on the establishment of prediction intervals. It is worth noting that while these methods have demonstrated utility, non-parametric approaches heavily depend on data abundance, whereas parametric methods are predominantly reliant on predefined data distributions \citep{wu2023adaptive,gawlikowski2021survey}.

% While parametric methods are generally preferred due to computational efficiency and adaptability, their application to sparse and event-centric spatiotemporal data is markedly limited \citep{jiang2023uncertainty}. \citet{zhuang2022uncertainty} and \citet{gao2023uncertainty} have introduced zero-inflated distributions in conjunction with spatiotemporal neural networks. This amalgamation was used to manage the prevalent zero instances and non-normal distribution found in sparse travel demand data. However, they confronted practical challenges when zero values were excessively extreme, especially in non-time series scenarios such as event-based risk situations, including traffic accidents and urban crime prediction. In these scenarios, the accuracy of predicting zeroes or non-zeroes significantly impacts the reliability and robustness of system design and monitoring. Consequently, the quantification and calibration of uncertainty within the sparsity component of spatiotemporal data is not only vital but also currently under-explored.

Spatiotemporal prediction through deep learning offers a powerful tool for various applications. Among them, GNNs have become prevalent in recent years \citep{wu2021inductive,zhao2022multi,yu2017spatio,wu2019graph}. Most existing models focus on predicting the deterministic values without considering the associated uncertainty, which leaves a noticeable research gap concerning UQ. Such a limitation impacts the reliability of predictions, as the unaccounted uncertainty can lead to deviations from the true data variance.

Bayesian and Frequentist approaches are the two main existing methods for spatiotemporal UQ \citep{wang2023uncertainty,zhou2021stuanet}. While the Bayesian approach offers profound insights through techniques like Laplace approximation \citep{wu2021bayesian}, Markov Chain Monte Carlo \citep{pearce2018high}, and Variational Inference \citep{khosravi2010lower}, it suffers from computational complexities and approximation inaccuracies. In contrast, the Frequentist approach exploits Mean-Variance Estimation for computational efficiency and model flexibility, accommodating both parametric and non-parametric methods \citep{wang2023uncertainty}. However, the application of these methods to sparse data is challenged by data dependencies and distribution constraints \citep{wu2023adaptive,gawlikowski2021survey}. For example, sparse data frequently deviate from models' mean-variance assumptions, favoring NB distributions over Gaussian, and traditional metrics like mean squared errors can be skewed by sparse datasets' non-zero values.
%sparse data often do not fit common models' mean-variance assumptions,

The use of zero-inflated distributions with spatiotemporal neural networks has been introduced to handle zero instances and non-normal distribution in sparse data \citep{zhuang2022uncertainty}. However, this approach has limitations in extreme scenarios and non-time-series contexts, impacting predictive accuracy and system robustness \citep{wang2023uncertainty,qian2023uncertainty}. Therefore, the urgent need to quantify and calibrate uncertainty in the sparse component of spatiotemporal data is evident, yet remains largely unexplored.

\subsection{Uncertainty Calibration}
Although relatively understudied in the spatiotemporal context, UQ has been examined by many machine learning studies. Among all the UQ approaches, calibration is a post-hoc method that aims to match the predictive probabilities of a model with the true probability of outcomes, developing robust mechanisms for uncertainty validation \citep{nixon2019measuring}.

Many techniques have been developed to calibrate pre-trained classifiers, mitigating the absence of inherent calibration in many uncertainty estimators \citep{kumar2019verified,gruber2022better,shen2023post}. Calibration for regression tasks, however, has received less attention \citep{thiagarajan2020building,kuleshov2018accurate}. Post-hoc calibration methods for classifications, such as temperature scaling, Platt scaling, and isotonic regression, have successfully been adapted for regression \citep{kull2019beyond}. Recent research \citep{chung2021beyond} further demonstrated quantile regression-based calibration methods and their extensions. These post-hoc methods offer greater flexibility and wider applicability to various probabilistic outputs compared to in-training methods, without necessitating model retraining \citep{rahman_uncertainty-aware_2023,huang_uncertainty_2023}.

In sparse spatiotemporal data contexts, where accurate model outputs are important for applications like traffic accident forecasting and crime prediction \citep{zhao2022multi}, the significance of uncertainty calibration is often overlooked. Traditional calibration methods focus on symmetric distributions like Gaussian, but sparse datasets commonly align with asymmetric NB distributions. Given the zero-inflated characteristics of such data, it is essential to discern confidence for zero and non-zero segments due to their varied implications. In response, we propose the SAUC method to manage asymmetric distributions and ensure empirical variances of true targets align with estimated PIs \citep{thiagarajan2020building}.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width= 0.8\textwidth ]{figs/models.pdf}
    \caption{Framework of models and experiments. We modify existing spatiotemporal GNNs into probabilistic ones with NB distribution parameters as the outputs. Sparsity-aware uncertainty calibration is then conducted to obtain the quantile regression results and calibrated confidence interval for forecasting. These two steps can be easily and practically generalized to all existing spatiotemporal GNNs.}
    \label{fig:model}
\end{figure*}

==> backup_KDD_sections/3.Preliminary.tex <==
\section{Problem Formulation}
% In this section, we introduce mathematical notations and problem formulations for the spatiotemporal prediction task and the associated uncertainty calibration process.

% Let $\mathcal{G} = (V,E,A)$ where $V$ represents the set of nodes (locations), $E$ the edge set, and $A\in \mathbb{R}^{|V|\times|V|}$ the adjacency matrix describing the relationship between nodes. Denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|V| \times t}$ where $t$ is the number of time steps. For simplicity, 

% The objective is to predict the value $y_{1:|V|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|V|,1:t}$. A predictive GNN model $f_{\theta}$, parametrized by $\theta$, generates the output $\hat{y}_{1:|V|,t:t+k} = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G})$. 

% With the emerging interest in probabilistic GNNs for discrete spatiotemporal predictions, the aim extends beyond mere predictions, seeking to capture the associated uncertainty, calling it UQ \citep{zhuang2022uncertainty,jiang2023uncertainty,wang2023uncertainty}. In our context, we assume each element $\hat{y}_{i,j}$ of model output $\hat{y}_{1:|V|,t:t+k}$ follows NB distribution characterized by shape parameter $\mu_{i,j}$ and dispersion parameter $\alpha_{i,j}$. The GNN model, in this probabilistic context, is then reformulated as follows:
% \begin{equation}
%     (\hat{\mu}_{1:|V|,t:t+k},\hat{\alpha}_{1:|V|,t:t+k}) = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G}).
% \end{equation}
% Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as delineated in Equation \ref{eq:modify_loss}.

\subsection{Spatiotemporal GNNs for Prediction} 
\noindent Let $\mathcal{G} = (\mathcal{V},\mathcal{E},\mathbf{A})$ where $\mathcal{V}$ represents the set of nodes (locations), $\mathcal{E}$ the edge set, and $\mathbf{A}\in \mathbb{R}^{|\mathcal{V}|\times|\mathcal{V}|}$ the adjacency matrix describing the relationship between nodes. We denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|\mathcal{V}| \times t}$ where $t$ is the number of time steps. The objective is to predict the target value $\mathcal{Y}_{1:|\mathcal{V}|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|\mathcal{V}|,1:t}$. The full dataset is partitioned by timesteps into training, calibration (i.e., validation), and testing sets. The three data partitions are denoted as $\mathcal{X}_{T}$, $\mathcal{X}_{S}$, and $\mathcal{X}_{U}$, respectively. For example, the training set $\mathcal{X}_{1:|\mathcal{V}|,1:t}$ is denoted as $\mathcal{X}_{T}$. The associated target values are represented as $\mathcal{Y}_{T}$, $\mathcal{Y}_{S}$,  and $\mathcal{Y}_{U}$, with subscripts indicating the corresponding sets.

The objective of the spatiotemporal GNN models is to design model $f_{\theta}$, parametrized by $\theta$, which yields:
\begin{equation}
    \hat{\mathcal{Y}}_d = f_{\theta}(\mathcal{X}_d; \mathcal{G}), \forall\ d \in \{ T,S,U \},
    \label{eq:GNN}
\end{equation}
where $\hat{\mathcal{Y}}_d$ is the predicted target value, and the subscript represents the corresponding data set. Note that $\theta$ is fixed once $f_{\theta}$ is trained on the set $T$.

With emerging interests in quantifying the data and model uncertainty of spatiotemporal GNNs, researchers shift towards designing probabilistic GNNs to predict both mean values and PIs \citep{wang2023uncertainty,bi2023mm}. Previous probabilistic spatiotemporal GNN studies often assume $\mathcal{X}$ and $\mathcal{Y}$ are independent and identically distributed NB random variables, i.e., $X_i$ and $Y_i$ for the sparse and discrete data \citep{zhuang2022uncertainty, jiang2023uncertainty}. The NB distribution of each predicted data point is characterized by shape parameter $\mu$ and dispersion parameter $\alpha$, and $\hat{\mu}_i \in \hat{M}_d$ denotes the mean value of the predicted distribution. Previous work has applied prediction layers with the corresponding likelihood loss after spatiotemporal GNN encoding to study the parameter sets of the predicted data points \citep{zhuang2022uncertainty,jiang2023uncertainty}. The set of predicted $\mu$ and $\alpha$ corresponding to all elements of $\mathcal{Y}$ are denoted as $\hat{M}$ and $\hat{H}$. Therefore, Equation \ref{eq:GNN} can be rewritten in the format of NB distribution-based probabilistic spatiotemporal GNNs as:
\begin{equation}
    (\hat{M}_d,\hat{H}_d) = f_{\theta} (\mathcal{X}_d; \mathcal{G}), \forall d \in \{ T,S,U \}.
    \label{eq:PGNN}
\end{equation}
Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as denoted in Equation \ref{eq:modify_loss}.

\subsection{Prediction Interval Calibration}
Uncertainty calibration refines the outputs of predictive models, such as GNNs, to ensure that predicted distributions accurately reflect the actual distributions. Traditionally, calibration methods presuppose that data follow a Gaussian distribution, characterized by mean and variance parameters. However, for sparse datasets, the NB distribution, which typically exhibits right skewness, is a more appropriate choice \citep{zhuang2022uncertainty}. Unlike the Gaussian distribution, where prediction interval widths are directly calculable from variance and z-scores, the NB distribution does not offer a simple expression for prediction intervals based on its parameters. Therefore, our calibration method aligns prediction intervals with data variance rather than modifying the NB distribution's parameters. This strategy builds upon and expands earlier research that prioritizes variance considerations.

The spatiotemporal prediction models output the sets of location and shape parameters $\hat{M}_d,\hat{H}_d, \forall d \in \{ T, S, U\}$. We then construct the prediction intervals of the $i$-th data point as $\hat{\mathcal{I}}_i = [\hat{l}_i,\hat{u}_i]$ with $\hat{l}_i$ and $\hat{u}_i$ denoting the 5th- and 95th-percentiles, respectively. Notably, our discussion limits the prediction intervals to the 5\% and 95\% range. Based on \citep{kuleshov2018accurate}, our target is to ensure a prediction model $f_{\theta}$ to be calibrated, i.e.,
\begin{equation}
    \frac{ \sum_{i=1}^{|U|} \mathbb{I}\{ y_{i} \leq \hat{F}_{i}^{-1}(p) \} }{|U|} \xrightarrow{|U| \rightarrow \infty} p,\  \forall p \in \{0.05, 0.95\},
    \label{eq:pi_calib}
% |V|\times k \rightarrow \infty
\end{equation}
where $p$ stands for the targeting probability values, $\mathbb{I}$ denotes the indicator function, and $\hat{F}_{i}(\cdot)$ is the CDF of the NB distributions parameterized by $\hat{\mu}_{i}$ and $\hat{\alpha}_{i}$. The primary goal is to ensure that, as the dataset size increases, the predicted CDF converges to the true one. Such an alignment is congruent with quantile definitions, suggesting, for instance, that 95\% of the genuine data should fall beneath the 95\% percentile. Rather than striving for a perfect match across $\forall p \in [0,1]$, we mainly focus on calibrating the lower bound and upper bound.

% \subsection{}
Empirically, we leverage the calibration set $S$ to calibrate the uncertainty in data. The empirical CDF for a given value $p \in \hat{F}_i (y_i)$ is computed \citep{kuleshov2018accurate,levi2022evaluating}:
\begin{equation}
    \hat{\mathcal{P}}(p) = \frac{ |\{ y_{i} | \hat{F}_i(y_i) \leq p, i = 1, \dots, |S| \} | }{|S|}.
    \label{eq:cdf}
\end{equation}
The calibration process entails mapping a calibration function $\mathcal{C}$, such as isotonic regression or Platt scaling, to the point set $\{ (p,\hat{\mathcal{P}}(p)) \}_{i=1}^{|S|} $. Consequently, the composition $\mathcal{C} \circ \hat{F}$ ensures that $\hat{\mathcal{P}}(p) = p$ within the calibration dataset. This composition can then be applied to the test set to enhance the reliability of predictions.



==> backup_KDD_sections/4.Methodology.tex <==
% \section{Methodology}
% In this section, we introduce mathematical notations, the general calibration process, and our proposed SAUC method. We first define the spatiotemporal prediction problem and then introduce the uncertainty calibration problem.


% % Let $\mathcal{G} = (V,E,A)$ where $V$ represents the set of nodes (locations), $E$ the edge set, and $A\in \mathbb{R}^{|V|\times|V|}$ the adjacency matrix describing the relationship between nodes. Denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|V| \times t}$ where $t$ is the number of time steps. For simplicity, 

% % The objective is to predict the value $y_{1:|V|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|V|,1:t}$. A predictive GNN model $f_{\theta}$, parametrized by $\theta$, generates the output $\hat{y}_{1:|V|,t:t+k} = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G})$. 

% % With the emerging interest in probabilistic GNNs for discrete spatiotemporal predictions, the aim extends beyond mere predictions, seeking to capture the associated uncertainty, calling it UQ \citep{zhuang2022uncertainty,jiang2023uncertainty,wang2023uncertainty}. In our context, we assume each element $\hat{y}_{i,j}$ of model output $\hat{y}_{1:|V|,t:t+k}$ follows NB distribution characterized by shape parameter $\mu_{i,j}$ and dispersion parameter $\alpha_{i,j}$. The GNN model, in this probabilistic context, is then reformulated as follows:
% % \begin{equation}
% %     (\hat{\mu}_{1:|V|,t:t+k},\hat{\alpha}_{1:|V|,t:t+k}) = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G}).
% % \end{equation}
% % Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as delineated in Equation \ref{eq:modify_loss}.



% \noindent\textbf{Spatiotemporal Prediction using GNNs.} Let $\mathcal{G} = (\mathcal{V},\mathcal{E},\mathbf{A})$ where $\mathcal{V}$ represents the set of nodes (locations), $\mathcal{E}$ the edge set, and $\mathbf{A}\in \mathbb{R}^{|\mathcal{V}|\times|\mathcal{V}|}$ the adjacency matrix describing the relationship between nodes. Denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|\mathcal{V}| \times t}$ where $t$ is the number of time steps. The objective is to predict the target value $\mathcal{Y}_{1:|\mathcal{V}|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|\mathcal{V}|,1:t}$. For the sake of clarity, and considering all nodes are incorporated into the analysis, we partition the dataset by timesteps into training, recalibration (i.e., validation), and testing sets. These datasets partitions are denoted by $\mathcal{X}_{T}$, $\mathcal{X}_{S}$,  and $\mathcal{X}_{U}$, respectively. For example, $\mathcal{X}_{1:|\mathcal{V}|,1:t}$ is denoted as $\mathcal{X}_{T}$. The associated target values are represented as $\mathcal{Y}_{T}$, $\mathcal{Y}_{S}$,  and $\mathcal{Y}_{U}$, with subscripts indicating the corresponding sets.

% The objective of the spatiotemporal GNN models is to design model $f_{\theta}$, parametrized by $\theta$, which yields:
% \begin{equation}
%     \hat{\mathcal{Y}}_d = f_{\theta}(\mathcal{X}_d; \mathcal{G}), \forall\ d \in \{ T,S,U \},
%     \label{eq:GNN}
% \end{equation}
% where $\hat{\mathcal{Y}}_d$ is the predicted target value, and the subscript represents the corresponding data set. Note that $\theta$ is fixed once $f_{\theta}$ is trained on set $T$.

% With the emerging interest in quantifying the data and model uncertainty of spatiotemporal GNNs, there is a shift towards utilizing probabilistic GNNs that predict not only mean values but also PIs \citep{zhuang2022uncertainty,jiang2023uncertainty,wang2023uncertainty}. In previous probabilistic spatiotemporal GNN studies, $\mathcal{X}$ and $\mathcal{Y}$ are assumed to consist of independent and identically distributed random variables $X$ and $Y$. In our study, $X$ and $Y$ are assumed to follow NB distributions when predicting discrete data. The NB distribution of each predicted data point is characterized by shape parameter $\mu$ and dispersion parameter $\alpha$. The set of predicted $\mu$ and $\alpha$ corresponding to all elements of $\mathcal{Y}$ are denoted as $\hat{M}$ and $\hat{H}$. Therefore, Equation \ref{eq:GNN} can be rewritten as:
% \begin{equation}
%     (\hat{M}_d,\hat{H}_d) = f_{\theta} (\mathcal{X}_d; \mathcal{G}), \forall d \in \{ T,S,U \}.
%     \label{eq:PGNN}
% \end{equation}
% Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as delineated in Equation \ref{eq:modify_loss}.

% \subsection{Problem Formulation}
% Uncertainty calibration aims to refine the outputs of prediction models (e.g., GNNs) such that the predicted distributions align with the true distributions. Traditional calibration models generally assume Gaussian distributions, which only involve the mean and variance parameters due to their intrinsic relationships with output variances, like the two-sigma associations. However, when dealing with discrete and sparse data, adopting alternative distributions such as the NB distribution is more suitable due to their asymmetric nature. Thus, our calibration methodology gives prominence to the prediction interval, serving as a natural extension of previous variance-oriented studies.

% From the spatiotemporal prediction model, with the outputs $\hat{M}_d,\hat{H}_d, \forall d \in \{ T, S, U\}$, we recognize $\hat{\mu}_i \in \hat{M}_d$ as the mean value of the predicted distribution of an individual future data point. We then use the 5\% to 95\% confidence interval of the output NB distributions as the prediction intervals $\hat{\mathcal{I}}_i = [\hat{l}_i,\hat{u}_i]$ with $\hat{l}_i$ and $\hat{u}_i$ denoting the lower and upper bounds, respectively. Notably, our discussion limits the prediction intervals to the 5\% and 95\% range. Based on \citet{kuleshov2018accurate}, our target is to ensure a prediction model $f_{\theta}$ to be calibrated, i.e.,
% \begin{equation}
%     \frac{ \sum_{i=1}^{|U|} \mathbb{I}\{ y_{i} \leq \hat{F}_{i}^{-1}(p) \} }{|U|} \xrightarrow{|U| \rightarrow \infty} p,\  \forall p \in \{.05, .95\},
%     \label{eq:pi_calib}
% % |V|\times k \rightarrow \infty
% \end{equation}
% where $p$ stands for the confidence level, $\mathbb{I}$ denotes the indicator function, and $\hat{F}_{i}(\cdot)$ is the cumulative density function (CDF) of the NB distributions steered by $\hat{\mu}_{i}$ and $\hat{\alpha}_{i}$. The primary goal is to ensure that, as the dataset size increases, the predicted CDF converges to the true one. Such an alignment is congruent with quantile definitions, suggesting, for instance, that 95\% of the genuine data should fall beneath the 95\% percentile. Rather than striving for a perfect match across $\forall p \in [0,1]$, we mainly focus on calibrating the lower bound and upper bound, mirroring earlier calibration endeavors centered around mean and variance.

% \subsection{Prediction-interval Based Calibration}
% For recalibrating the uncertainty inherent in our prediction model, we leverage the model's output for the recalibration set $S$. The empirical CDF for a given predicted CDF value $p \in \hat{F}_i (y_i)$  is then computed \citep{kuleshov2018accurate,levi2022evaluating}:
% \begin{equation}
%     \hat{\mathcal{P}}(p) = \frac{ |\{ y_{i} | \hat{F}_i(y_i) \leq p, i = 1, \dots, |S| \} | }{|S|}.
%     \label{eq:cdf}
% \end{equation}
% The calibration process entails mapping a calibration function $\mathcal{C}$, such as isotonic regression or Platt scaling, to the point set $\{ (p,\hat{\mathcal{P}}(p)) \}_{i=1}^{|S|} $. Consequently, the composition $\mathcal{C} \circ \hat{F}$ ensures that $\hat{\mathcal{P}}(p) = p$ within the recalibration dataset. This composition can then be extended to the prediction outputs on the test set for enhanced reliability.


\section{Sparsity-Aware Uncertainty Calibration}

\subsection{QR for Uncertainty Calibration}
\label{sec:qr}
%QR excels in modeling the conditional quantiles of a response variable, elevating its significance for uncertainty calibration. 
Unlike traditional regression techniques that target the conditional mean, QR predicts specific quantiles, which are essential for calibrating PIs. Given $\hat{M}_S$ and $\mathcal{Y}_S$ from the calibration set $S$, the linear QR model can be expressed as:
\begin{equation}
    Q_{\mathcal{Y}_S | \hat{M}_S }(p) = \hat{M}_S^T \beta(p),
    \label{eq:QR}
\end{equation}
where $\beta(p)$ signifies the coefficient associated with quantile $p$. The goal here is to minimize the Pinball loss \citep{chung2021beyond}, which is defined as: 

\begin{equation}
L_{\text{pinball}}(y, \hat{y}, p) =
\begin{cases}
(p-1) \cdot (y - \hat{y}), & \text{if } y < \hat{y} \\
p \cdot (y - \hat{y}), & \text{if } y \geq \hat{y}
\end{cases}.
\end{equation}
In our context, we focus on the cases of $p=5\%$ and 95\%, and thus the quantile regressions output calibrated PIs correspond to $[Q(0.05),Q(0.95)]$.

While the NB distribution is frequently used for estimating sparse data uncertainty, it can still be prone to mis-specification, particularly when assumptions about data characteristics are less precise \citep{zhuang2022uncertainty,jiang2023uncertainty,sankararaman2013distribution}. In such instances, non-parametric (not directly modeling the distribution parameters) methods like QR emerge as robust alternatives, compared to a direct scaling or fitting of the dispersion parameter \citep{laves2020well,bishop2006pattern}. QR's resilience to data assumptions helps mitigate potential errors in model specification, a critical advantage especially in handling datasets with heavy tails where significant risks or events are concentrated—features sometimes not fully captured by parametric models \citep{hao2007quantile}. 

QR is also adept at addressing heteroscedasticity, where variance shifts with the response variable, a situation often oversimplified by a single dispersion parameter in parametric calibration models \citep{zheng2018hybrid,antunes2017review}. Its ability to handle sparse datasets and accommodate variance fluctuations, particularly in scenarios with numerous zeros, further underscores its utility. Enhanced with basis expansion techniques, QR can discern complex patterns across various quantiles, making it an ideal choice for scenarios where zero outcomes are prevalent and a nuanced understanding of data patterns and risks is crucial.

\subsection{SAUC Method}
Our SAUC method is a two-step post-hoc nonparametric calibration method tailored for sparse data, as detailed in Figure \ref{fig:model}. In the training phase, we trained the modified NB-based probabilistic spatiotemporal GNNs to obtain the model parameters $\theta$ (modifications detailed later). In the calibration phase, this training yields $\hat{M}_S,\hat{H}_S$ on the calibration set for uncertainty calibration. Drawing inspiration from zero-inflated models, predictions in the calibration set $S$ are bifurcated based on \textbf{indices}: $I_{Z} = \{\hat{M}_S < 0.5\}$ for prediction values nearing zero, and $I_{NZ} = \{\hat{M}_S \geq 0.5\}$ for non-zero predictions. The value of 0.5 is a natural dividing line for the rounding operations to determine if values are effectively zeroes. Following this partitioning, two QR models, $Q_Z$ and $Q_{NZ}$, are trained separately, calibrating quantiles $p = \{ .05, .95 \}$ to fine-tune the mean and PI predictions. The calibrated model is then applied to predict model outputs on the testing set. Pseudocode details for implementing the SAUC method are provided in Algorithm \ref{alg:sauc}, and codes can be found in the anonymous GitHub repository \footnote{\url{https://github.com/AnonymousSAUC/SAUC}}.

The SAUC method focuses on calibrating PIs rather than modifying distribution parameters, aligning with the principles of previous post-hoc calibration methods like isotonic regression and Platt scaling \citep{niculescu2005predicting,kuleshov2018accurate}. These methods are designed to refine a model's outputs without directly altering internal parameters such as the parameters $\mu$ and $\alpha$ of NB distributions. This strategy ensures a distinct separation between modeling and calibration, enhancing flexibility and broad applicability. It avoids complicating the calibration process and potentially impacting the core modeling objectives. Additionally, post-hoc methods have demonstrated practical effectiveness and computational efficiency in improving the probabilistic accuracy of predictions, without necessitating retraining or modifications to the original model.

\begin{algorithm}[t]
\caption{SAUC Method}
\begin{algorithmic}[1]
\REQUIRE $\hat{M}_S$, $\mathcal{Y}_S$, $N$, $\hat{M}_U$, $p\leftarrow \{ .05, .95 \}$
\STATE Define the bin thresholds $\mathcal{T}_S$ using percentiles of $\mathcal{Y}_S$.
\STATE Initialize $U^*$, $L^*$ in the same size as $\hat{M}_U$.
\FOR{each bin $i$ in $[1, N]$}
\STATE Extract indices $I$ of instances in bin $i$ based on $\mathcal{T}_S$.
\STATE Split $I$ to $I_{NZ}$ for $\hat{M}_S\geq 0.5$ and $I_Z$ for $\hat{M}_S<0.5$.
\FOR{each set $i$ in $\{I_{NZ}, I_Z\}$}
\FOR{each value $q$ in $p$}
\STATE Fit $Q(q)$ on $\hat{M}_S[i]$ and $\mathcal{Y}_S[i]$ based on Equation \ref{eq:QR} and obtain $\beta (q)$.
\ENDFOR
\STATE 
% $M^*[i]\leftarrow \hat{M}_U^T \beta(.5)$,
$L^*[i]\leftarrow \hat{M}_U^T \beta(.05)$, $U^*[i]\leftarrow \hat{M}_U^T \beta(.95)$
\ENDFOR
\ENDFOR
\STATE $\mathcal{I}^* \leftarrow [L^*, U^*] $.
\RETURN $\mathcal{I}^*$.
\end{algorithmic}
\label{alg:sauc}
\end{algorithm}

% In the proposed SAUC method, special emphasis is given to local calibrations, particularly addressing data sparsity. While \citet{song2019distribution} have highlighted that a quantile-calibrated regression model offering predictions with specific empirical moments (e.g. mean and variance) does not ensure that targets with identical predicted moments universally maintain the same true moments, this is largely because traditional approaches contemplate the issue on a broad scale, calibrating quantiles globally. However, by partitioning the data into zero and non-zero segments, our method is designed to obtain nuanced quantile calibrations for these distinct components, each bearing unique implications. The zero segment, potentially substantial in size, necessitates meticulous calibration due to its binary nature in practical scenarios. Conversely, for the non-zero section, it's vital that predicted quantiles genuinely represent the actual event quantiles, as research in this domain typically seeks to interpret relative risks or event severities.

\citep{song2019distribution} argued that quantile regressions might not retain true moments for the targets with similar predicted moments because of the global averaging effects. Our SAUC method addresses this limitation because it creates local segments based on zero and non-zero values. The zero segment, potentially dominant, requires precision in calibration due to its binary implications in real-world applications. For the non-zero subset, the aim is to ensure that quantiles mirror actual event frequencies, resonating with the typical research focus on discerning relative risks or magnitudes of events. Notice that even though our SAUC method is discussed based on Equation \ref{eq:PGNN} in GNN models, it can be generalized to any spatiotemporal prediction task.

\subsection{Calibration Metrics for Asymmetric Distributions}

While calibration errors are clearly established for classification tasks using Expected Calibration Error \citep{nixon2019measuring,gruber2022better,kumar2019verified}, the definition is much less studied in the regression context, where prediction errors and intervals supersede accuracy and confidence. Based on Equation~\ref{eq:pi_calib} and~\ref{eq:cdf}, we aim to calibrate the length of the prediction interval with the standard error, i.e.,
\begin{equation}
    \small
    \big[\mathbb{E}[ (\hat{\mu}_i - Y_i)^2 | \hat{\mathcal{I}_i} = \mathcal{I}_i ]\big]^{1/2} = c|\mathcal{I}_i|, \ \forall i \in \{ 1, \dots, |U| \}.
    \label{eq:define_calib}
\end{equation}
Note that $\mathcal{I}_i= [F_i^{-1}(.05),F_i^{-1}(.95)]$ is the realization of the predicted 5\%-95\% confidence interval and $|\mathcal{I}_i|$ denotes its width. Calibrating the model's standard errors with the 90\% confidence interval width reveals a linear relationship with coefficient $c$, specifically for symmetric distributions like Gaussian. As an approximation, we continue to use the z-score of Gaussian distribution to compute the coefficient $c$. The width of 5\%-95\% confidence interval is roughly $2\times 1.645 = 3.29$ of the standard error, inversely proportional to $c$. Empirical results, illustrated in Figure \ref{fig:find_c}, support a linear correlation between the ratio of the predicted interval $\hat{\mathcal{I}}$ and the estimated standard error of the distribution. In our experiments, this slope ranges from 0.3 to 0.4, aligning closely with our theoretical assumption. Consequently, this leads to a value of $c \approx \frac{1}{3.29} \approx 0.303$.


\begin{figure}[t!]
    \centering    \includegraphics[width=0.8\linewidth]{figs/find_c.pdf}
    \vspace{-1em}
    \caption{Explore the linear correlation between MPIW and RMSE using different cases of the CCR data.}    
    \label{fig:find_c}
\end{figure}

Therefore, we could diagnose the calibration performance by comparing value differences on both sides of the equation. Specifically, we partition the \textbf{indices} of test set samples into $N$ evenly sized bins based on sorted predicted PI width, denoted as $\{B_j\}_{j=1}^N$. In our study, we set $N=15$ by default. Each bin corresponds to a PI width that falls within the intervals: $[\min_{i\in B_j}\{ |\mathcal{I}_i| \}, \max_{i\in B_j}\{ |\mathcal{I}_i| \}]$. Note that the intervals are non-overlapping and their boundary values are increasing. Based on the discussion of \citet{levi2022evaluating} and Equation \ref{eq:define_calib}, for $j$-th bin, we define the Expected Normalized Calibration Error (ENCE) based on Root Mean Squared Error (RMSE) and Mean Prediction Interval Width (MPIW):
\begin{equation}
ENCE = \frac{1}{N} \sum_{j=1}^N \frac{|c \cdot MPIW(j) -  RMSE(j) |}{c \cdot MPIW(j)},
\label{eq:ence}
\end{equation}
where the $RMSE$ and $MPIW$ are defined as:
\begin{align}
    RMSE(j) &= \sqrt{ \frac{1}{|B_j|} \sum_{i\in B_j} (\hat{\mu}_i - y_i)^2 }\\
    MPIW(j) &= \frac{1}{|B_j|} \sum_{i \in B_j} |\hat{\mathcal{I}}_i|
\end{align}

The proposed ENCE normalizes calibration errors across bins, sorted and divided by $c \cdot MPIW$, and is particularly beneficial when comparing different temporal resolutions and output magnitudes across datasets. The $c \cdot MPIW$ and observed $RMSE$ per bin should be approximately equal in a calibrated forecaster.



==> backup_KDD_sections/5.Experiments.tex <==
\section{Experiments}


% \begin{table*}[!t]
%     \scriptsize
%     \centering    
%     \begin{tabularx}{\linewidth}{c*{7}{>{\centering\arraybackslash}X}@{\hspace{4pt}}c@{\hspace{4pt}}*{7}{>{\centering\arraybackslash}X}}
%     \toprule
%     \multicolumn{16}{c}{STGCN-NB Outputs} \\
%     \hline
%     {} & \multicolumn{7}{c}{Full observations} & \vline & \multicolumn{7}{c}{Sparsity-entry only} \\
%     \hline
%     Method & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
%     Interval    &  calibration    &  binning         &   regression       &   scaling   &    scaling &     &             &    \vline &  calibration        &      binning     &     regression     &          scaling  &    scaling    &   &         \\
%     \midrule
%     CCR\_1h       &        0.217 &     0.199 &    0.207 &    0.215  &  0.185 &  \underline{0.164}  &   \textbf{0.160} &       \vline & 0.524 &     0.189 &    \underline{0.129} &     0.500 &  0.362 &  0.269 & \textbf{0.001}     \\
%     CCR\_8h       &        0.315 &     0.097 &    \textbf{0.048} &     0.241 &  0.210 &    0.312   &\underline{0.109} &     \vline &   0.208 &     0.159 &    0.226 &     0.303 &  \underline{0.062} &  0.336 & \textbf{0.052}     \\
%     CCR\_1d    &        0.505 &     \underline{0.238} &    \textbf{0.185} &     0.468 &  0.873 & 0.330 &      0.275  &       \vline & 0.991 &     0.977 &    0.732 &     0.868 &  \textbf{0.208} &  0.330  & \underline{0.284}    \\
%     CCR\_1w       &        0.415 &     \underline{0.403} &     0.414&     0.416 &  1.965 & 0.260 & \textbf{0.342}      &     \vline &   0.145 &     1.084 &    0.143 &     \underline{0.105} &  0.151 &  0.108 & \textbf{0.058}    \\
    
%     \midrule
%     CTC\_1h       &        0.082 &     0.214 &    0.210 &       \underline{0.114}  &  0.163 &  0.048 &  \textbf{0.028} &      \vline &  0.042 &     0.702 &    0.579 &    0.381 &  0.596 & \underline{0.006} & \textbf{ 0.005}      \\
%     CTC\_8h       &        0.189 &     0.200 &    0.136 &       0.211 &  \underline{0.079} &  0.163  & \textbf{0.040}   &     \vline &   0.213 &     0.226 &    \underline{0.131} &     0.255 &  0.168 &  0.179 & \textbf{0.003}      \\
%     CTC\_1d    &        0.303 &     \underline{0.075} &    \textbf{0.060} &   0.422 & 0.265  &  0.170 &    0.079   &      \vline &  0.007 &     0.154 &    \underline{0.078} &     0.537 &  0.240 &  0.152 & \textbf{0.002}     \\
%     CTC\_1w       &        1.482 &     0.850 &    1.048 &     \underline{0.833} &  1.596 & 0.955 & \textbf{0.225}      &    \vline &    0.814 &     1.447 &    1.237 &     \underline{0.754} &  0.958 &  0.846 & \textbf{0.196}     \\

%     % \midrule
%     % SLD\_5min & & & & & & & & & & & & \\
%     % SLD\_15min & & & & & & & & & & & & \\
%     % SLD\_60min & & & & & & & & & & & & \\
%     \hline
%     \multicolumn{16}{c}{GWN-NB Outputs} \\
%     \hline
%     {} & \multicolumn{7}{c}{Full observations} & \vline & \multicolumn{7}{c}{Sparsity-entry only} \\
%     \hline
%     Method & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
%     Interval    &  calibration    &  binning         &   regression       &   scaling   &    scaling    &    &           &      \vline & calibration        &      binning     &     regression     &          scaling  &    scaling    &     &         \\
%     \midrule
%     CCR\_1h       &        0.904 &     0.796 &    0.838 &       1.978 &  0.769 &  \underline{0.220}   &\textbf{0.199} &       \vline &  0.377 &     0.451 &    0.658 &       0.378 &  0.322 &  \underline{0.211}  & \textbf{0.001} \\
%     CCR\_8h       &        2.585 &     0.640 &    0.618 &       1.257 &  \underline{0.415} &  0.483   &\textbf{0.378} &    \vline &    0.686 &     \underline{0.138} &    0.180 &       0.440 &  0.187 & 0.354    &\textbf{0.043} \\
%     CCR\_1d     &   1.186 &     0.883 &    1.024 &       3.270 &  1.006 &  \underline{0.427}   &\textbf{0.352}  &   \vline &     1.540 &     0.528 &    0.652 &       1.537 &  \underline{0.425} &  0.639   &\textbf{0.115} \\
%     CCR\_1w       &        2.990 &     0.384 &    \underline{0.307} &       2.503 &  \textbf{0.211} &  2.030  & 0.330 &    \vline &    3.736 &     0.387 &    \textbf{0.356} &       3.737 &  0.534 &  1.911  & \underline{0.308} \\
    
%     \midrule
%     CTC\_1h      & 0.381 & 0.355 & 0.341 & 0.334 &  0.434 & \underline{0.222} &\textbf{0.186} & \vline & 0.784 & 0.641 & 0.610 &       0.784 &  1.000 &  \underline{0.105} &\textbf{0.003} \\
%     CTC\_8h      & 0.931 & 0.416 &  0.388 & 1.381 &  \underline{0.169} & 0.226  &\textbf{0.148} &        \vline & 2.213 &     0.720 &    0.659 &       1.995 &  \underline{0.421} &  0.776   &\textbf{0.221}\\
%     CTC\_1d      & 0.523 & \underline{0.420} & 0.448 & 0.571 &  0.523 & 0.432   &\textbf{0.139}  &        \vline & 0.250 &     0.464 &    0.405 &       \underline{0.248} &  0.484 &   0.439  &\textbf{0.010} \\
%     CTC\_1w      & 0.408 & 0.114 & \underline{0.114} & 0.259 &  0.236 & 0.241 &\textbf{0.090} &        \vline & 0.466 &     0.479 &    \underline{0.436} &       0.457 &  0.451 &  0.476  &\textbf{ 0.350}\\
    
%     % \midrule
%     % SLD\_5min  & & & & & & & & & & & & \\
%     % SLD\_15min & & & & & & & & & & & & \\
%     % SLD\_60min & & & & & & & & & & & & \\
%     \bottomrule
%     \end{tabularx}
%     \caption{ENCE of the different calibration models. Bold fonts mark the best and underlines denote the second-best calibration models.}
%     \label{tab:ce_full}
% \end{table*}


\subsection{Data Description}
Two spatiotemporal datasets are used: (1) Chicago Traffic Crash Data (CTC) sourced from 277 police beats between January 1, 2016 and January 1, 2023; (2) Chicago Crime Records (CCR) derived from 77 census tracts spanning January 1, 2003 to January 1, 2023. Despite both CTC and CCR data originating from the Chicago area, their disparate reporting sources lead to different spatial units: census tracts for CCR and police beats for CTC. Both datasets use the first 60\% timesteps for training, 20\% for calibration and validation, and 20\% for testing.

% The temporal resolutions of the datasets are varied to demonstrate the ubiquitous sparsity issue and its practical significance in spatiotemporal analysis. For example, four temporal resolutions are created for CTC and CCR datasets, with details available in Table \ref{tab:data_sparsity}. We designate the 1-hour and 8-hour cases of Crash and Crime datasets as sparse instances, due to a higher prevalence of zeros.

To highlight the prevalent sparsity issue in spatiotemporal analysis, we varied the temporal resolutions of the CTC and CCR datasets, as detailed in Table \ref{tab:data_sparsity}. Specifically, we classified the 1-hour and 8-hour intervals in the CTC and CCR datasets as sparse due to their significantly higher zero counts. The histogram in Figure \ref{fig:sparsity_transition} further demonstrates this concept, showing traffic crash counts in all police beats across different temporal resolutions. Notably, higher resolutions show noticeable skewness and clustering of values at lower counts, illustrating the sporadic nature of traffic incidents. This observation emphasizes the importance of equipping predictive models with capabilities to adeptly manage sparse data, thereby more accurately mirroring real-world temporal patterns.

\begin{table}[t]
    \small
    \centering
    \begin{tabular}{cc|cc}
    \toprule
        Dataset & Temporal resolution  & Size & Sparsity\\
    \midrule              
       \multirow{4}{*}{CCR}  & \cellcolor{Gray}1-hour & \cellcolor{Gray}(77, 175321)& \cellcolor{Gray}67\%\\
       & \cellcolor{Gray}8-hour & \cellcolor{Gray}(77, 21916) & \cellcolor{Gray}18\%\\
       & 1-day  & (77, 7306)  & 4\%\\ 
       & 1-week & (77, 1044)& $<0.1\%$\\
    \midrule
       \multirow{4}{*}{CTC}  & \cellcolor{Gray}1-hour & \cellcolor{Gray}(277, 61369) & \cellcolor{Gray}96\% \\   
       & \cellcolor{Gray}8-hour & \cellcolor{Gray}(277, 7672) & \cellcolor{Gray}76\% \\
       & 1-day  & (277, 2558) & 47\% \\
       & 1-week & (277, 366) & 7\% \\
    % \midrule        
    %       \multirow{3}{*}{SLD}  & \cellcolor{Gray}5min  &  \cellcolor{Gray}(4489, 34560) & \cellcolor{Gray}88\% \\
    %       & 15min &  (4489, 11520) & 70\% \\
    %       & 60min &  (4489, 2880)  & 50\% \\          
    \bottomrule
    \end{tabular}
    \caption{Characteristics of various datasets showing variation in sparsity at different temporal resolutions. Dataset sizes are represented as (spatial, temporal) dimension pairs. Sparse cases are marked grey.}
    \label{tab:data_sparsity}
\end{table}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/sparsity_transition_hist.pdf}
    \vspace{-1em}
    \caption{Histogram of number traffic crashes in the CTC data in different temporal resolutions}
   \label{fig:sparsity_transition}
\end{figure}

For adjacency matrices, we calculate geographical distances $d_{ij}$ between the centroids of regions $i$ and $j$, representing census tracts or police beats. This distance is then transformed into a similarity measure, $\mathbf{A}_{ij} = e^{-d_{ij}/0.1}$, where $0.1$ is a scaling parameter, thus forming an adjacency matrix \citep{yu2017spatio}.

\subsection{Modified Spatiotemporal Models}
In order to demonstrate our model's ability to generalize on spatiotemporal prediction models, we modify three existing popular spatiotemporal forecasting models: Spatio-temporal Graph Convolution Network (STGCN) \citep{yu2017spatio}, Graph WaveNet (GWN) \citep{wu2019graph}, and Dynamic Spatial-Temporal Aware Graph Neural Network (DSTAGNN) \citep{lan2022dstagnn}. They are designed for numerical value outputs. We modify their last layer from single numerical output to the location parameter $\mu$ and the dispersion parameter $\alpha$ of negative binomial distributions. Two linear layers are added at the end of the neural network structures to learn the parameters. We renamed the modified model as STGCN-NB, GWN-NB, and DSTAGNN-NB, respectively. Besides, we modify the loss function from mean square error loss to the likelihood loss defined in Equation \ref{eq:modify_loss}:
\begin{equation}
\begin{aligned}
& \mathcal{L}(\mu, \alpha, y) = -\left[y \cdot \log\left(\frac{\mu + \epsilon}{\mu + \alpha + 2\epsilon}\right)\right] \\
&\quad\quad - \Gamma(y + \alpha + \epsilon) + \Gamma(y + 1) + \Gamma(\alpha + \epsilon) \\
&\quad\quad - \alpha \cdot \log\left(\frac{\alpha + \epsilon}{\mu + \alpha + 2\epsilon}\right) + \lambda \cdot ||\alpha||^2
\label{eq:modify_loss}
\end{aligned},
\end{equation}
where $y$ is the target variable, $\mu$ and $\alpha$ are model outputs, $\Gamma$ is the gamma function, $\lambda$ is the regularization parameter, and $\epsilon$ is a small constant added to improve numerical stability. Equation \ref{eq:modify_loss} is derived from the NB likelihood controlled by $\mu$ and $\alpha$.

The loss function ensures the predicted NB distribution aligns well with the true target values. It penalizes predictions where the mean of the distribution ($\mu$) is far from the actual target values. Furthermore, it incorporates the shape of the distribution via the dispersion parameter ($\alpha$) to capture the variability in the data. The loss function also includes a regularization term to prevent overfitting by discouraging overly large values of $\alpha$.

\begin{table}[!h]
    \small
    \centering
    \begin{tabular}{cccc}
    \toprule
        Dataset & STGCN & GWN & DSTAGNN \\
    \midrule              
        CCR\_1h & 0.637 (0.703) & 0.962 (0.766) & 1.226 (1.117)\\
        CCR\_8h & 2.386 (2.326) & 2.052 (2.376) & 2.272 (2.693)\\
        CTC\_1h & 0.214 (0.220) & 0.980 (0.220) & 1.074 (0.871)\\
        CTC\_8h & 0.633 (0.726) & 0.924 (0.746) & 1.289 (1.177)\\
    \bottomrule
    \end{tabular}
    \caption{RMSE of original model outputs and the modified models (shown in the parenthesis) using sparse datasets.}
    \label{tab:model_modification}
\end{table}
\vspace{-1em}

As shown in Table \ref{tab:model_modification}, the model modification is successful without losing accuracy. In fact, the NB modification performs better in the sparse dataset as the NB distributions are more suitable for the nature of discrete data. 


% Detailed numerical comparisons can be found in \redfont{Appendix}.




% excluding calibration techniques that incorporate uncertainty during training \citep{thiagarajan2020building,huang_uncertainty_2023}
\setlength{\dbltextfloatsep}{1pt} %
\begin{table*}[!ht]
    \scriptsize
    \centering 
    \begin{tabularx}{0.98\linewidth}{c*{7}{>{\centering\arraybackslash}X}@{\hspace{4pt}}c@{\hspace{4pt}}*{7}{>{\centering\arraybackslash}X}}
    \toprule
    {} & \multicolumn{7}{c}{Full observations} &  & \multicolumn{7}{c}{Zero-only targets} \\ 
    \midrule
    
    Method / & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
    Dataset    &  calibration    &  binning         &   regression       &   scaling   &    scaling &     &             &    \vline &  calibration        &      binning     &     regression     &          scaling  &    scaling    &   &         \\
    \midrule
    \multicolumn{16}{c}{\textbf{STGCN-NB Outputs}} \\   
    \midrule
    CCR\_1h       &     1.160 &     0.410 &    0.517 &    0.887     &  0.443  &   \underline{0.235}  & \textbf{0.198}  &    \vline  &   1.167 &     0.361 &  0.386   &   0.473   &  0.477 &  \underline{0.273} &  \textbf{0.267}  \\
    CCR\_8h       &   1.389 &   \underline{0.344}   &    0.417 &    0.385  &  0.373 &  0.392 &  \textbf{0.336}    &  \vline  &   1.065 &     0.568 &    0.578 &       0.427 &  \underline{0.162} &  0.175  & \textbf{0.127}  \\
    CCR\_1d       &    0.413 &     0.593 &    0.546 &       0.364 &  \underline{0.294} &  0.297  &  \textbf{0.192}   &  \vline  &  1.266 &     1.047 &    0.979 &       1.167 &  \underline{0.840}  &    0.843    &  \textbf{0.738} \\
    CCR\_1w       &   0.855 &     0.784 &    0.773 &       0.765 &  0.579 & \underline{0.272} &    \textbf{0.242}   &    \vline  &   0.354 &     0.362 &    0.332 &       0.287 &  0.345 &  \underline{0.155}  &  \textbf{0.113}  \\    
    \midrule
    CTC\_1h       &    0.578 &     0.227 &    \underline{0.200} &       1.390 &  0.452 &  0.388 &   \textbf{0.165}  &       \vline  &   3.211 &     0.415 &    \underline{0.363} &       2.042 & 0.646 &  0.416  &   \textbf{0.078} \\
    CTC\_8h       &   0.323 &     0.320 &    0.255 &       0.570 &  0.297 &  \underline{0.241}  &  \textbf{0.233}   &       \vline  &  0.330 &     0.247 &    0.276 &       0.551 &  0.230 &  \underline{0.196}  &  \textbf{0.184} \\
    CTC\_1d       &   0.722 &     0.050 &     \textbf{0.011}  &       0.862 &  0.060 &  0.048  &  \underline{0.047} &       \vline  &  0.434 &     0.128 &    \textbf{0.027} &       5.451 &  0.152 &  0.379  & \underline{0.150}  \\
    CTC\_1w       &     2.279 &     1.227 &    1.527 &       0.914 &  2.265 &  \underline{0.378}   & \textbf{0.365} &       \vline  &  1.823 &     2.384 &    2.009 &       1.160 &  1.343 &  \underline{0.767}  &  \textbf{0.755}  \\

    % \midrule
    % SLD\_5min & & & & & & & & & & & & \\
    % SLD\_15min & & & & & & & & & & & & \\
    % SLD\_60min & & & & & & & & & & & & \\
    \midrule
    \multicolumn{16}{c}{\textbf{GWN-NB Outputs}} \\
    % \hline
    % {} & \multicolumn{7}{c}{Full observations} & \vline & \multicolumn{7}{c}{Zero-only targets} \\
    % \hline
    % Method / & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
    % Interval    &  calibration    &  binning         &   regression       &   scaling   &    scaling    &    &           &      \vline & calibration        &      binning     &     regression     &          scaling  &    scaling    &     &         \\
    \midrule
    CCR\_1h       &  1.200 &     1.022 &   0.889   &   1.149   &  0.834 & \underline{0.604}  & \textbf{0.493}   &   \vline  &  2.042 &     1.796 &    1.274 &       1.710 &  1.356 &  \underline{0.476}  &  \textbf{0.375} \\
    CCR\_8h       &    0.670 &     0.636 &    0.612 &   0.696 &  0.655 &  \underline{0.597} & \textbf{0.566}   &       \vline  &  1.398 &     0.389 &    0.492 &    1.179    &  0.478 &  \underline{0.308}   &  \textbf{0.186}   \\
    CCR\_1d       &   0.997  &     0.662 &    0.633 &    0.581 &  \underline{0.562} & 0.587  &  \textbf{0.504} &       \vline  &  1.158 &     0.583 &    \underline{0.580} &       0.725 &  0.747 &  0.644  & \textbf{0.563}  \\
    CCR\_1w       &    0.858 &     0.938 &    0.935 &       \textbf{0.611} &  0.931 &  0.857 &  \underline{0.829}  &       \vline  &  0.335 &     0.218 &    0.219 &       \textbf{0.161} &  0.219 & 0.250  &  \underline{0.172}    \\
    
    \midrule
    CTC\_1h      &   0.868  &  0.816  &  0.891  &  0.859  & \underline{0.634}  &  0.832  &  \textbf{0.290}  &  \vline  & 1.300  &  0.712  &  0.561  & 1.001  &  \underline{0.143}  &  0.998  & \textbf{0.139}  \\
    CTC\_8h      & 0.931 & 0.416 &  0.388 & 1.381 &  \underline{0.169} & 0.226  &\textbf{0.148} &        \vline & 2.213 &     0.720 &    0.659 &       1.995 &  \underline{0.421} &  0.776   &\textbf{0.221}\\
    CTC\_1d      & 0.523 & \underline{0.420} & 0.448 & 0.571 &  0.523 & 0.432   &\textbf{0.139}  &        \vline & 0.250 &     0.464 &    0.405 &       \underline{0.248} &  0.484 &   0.439  &\textbf{0.210} \\
    CTC\_1w      & 0.408 & 0.115 & \textbf{0.114} & 0.259 &  \underline{0.236} & 0.241 &0.239 &        \vline & 0.466 &     0.479 &    \textbf{0.436} &       0.457 &  0.451 &  0.476  & \underline{0.450}\\
    
    \midrule
    \multicolumn{16}{c}{\textbf{DSTAGNN-NB Outputs}} \\
    \midrule
    CCR\_1h     & 0.328 &     0.695  &    0.695 &       0.958 &  0.667 & \underline{0.230} &    \textbf{0.107} &  \vline  & 0.292 &     0.773 &    0.752 &       4.853 &  0.900 &  \underline{0.120}  & \textbf{0.102}\\
    CCR\_8h      &    0.895 &     0.941 &    0.940 &       0.604 &  0.928 &  \underline{0.443}  &  \textbf{0.440}  & \vline  &         0.811 &     0.905 &    0.901 &       \underline{0.419} &  0.930 & 0.572  &  \textbf{0.314} \\
    CCR\_1d       &  0.962 &     0.950 &    0.950 &       0.810 &  0.946 & \underline{0.792}  &   \textbf{0.709} &  \vline  &  0.822 &     0.790 &    0.788 &       0.619 &  0.797 &  \underline{0.235}  & \textbf{0.171} \\
    CCR\_1w        &   0.999 &     1.000 &    1.000 &       0.987 &  1.000 &  \underline{0.977} &   \textbf{0.952}   &  \vline  &  0.260  &     0.140 &    0.140 &       \textbf{0.138} &  \underline{0.139} & 0.150 &  0.149 \\
    
    \midrule
    CTC\_1h     &    0.398 &     0.187 &    \underline{0.121} &     0.138 &  0.129 & 0.159 & \textbf{0.119} &  \vline  & 0.937 &     0.652 &    0.661 &     1.222 &  0.970 & \underline{0.631} & \textbf{0.229} \\
    CTC\_8h       &   1.462 &     0.666 &    0.669 &      \underline{0.473} &  0.767 & 0.505 & \textbf{0.452} & \vline  & 0.694 &     \underline{0.575} &    0.608 &       0.586 &  0.950 & 0.612 & \textbf{0.523} \\
    CTC\_1d     &   1.393 &     0.776 &    0.774 &       1.304 &  0.725 & \underline{0.481} &  \textbf{0.402} &  \vline  & 1.650 &     0.789 &    0.771 &       1.259 &  1.000 & \underline{0.637} & \textbf{0.503}  \\
    CTC\_1w       & 0.890 &     0.876 &    0.874 &       \textbf{0.717} &  0.840 &   \underline{0.824} & 0.833  & \vline  &  0.980 &     0.757 &    0.743 &       \textbf{0.498} &  0.827 & 0.679 &  \underline{0.550}\\
    \bottomrule
    \end{tabularx}
    \caption{ENCE of the calibration models. Bold fonts mark the best and underlines denote the second-best calibration results.}
    \label{tab:ce_full}
\end{table*}


\subsection{Baseline Calibration Methods}
We compare the SAUC method with existing post-hoc calibration methods proven to be effective in the regression tasks:
(1) \textit{Isotonic regression} \citep{niculescu2005predicting}, which ensures non-decreasing predictive probabilities, assuming higher model accuracy with increased predicted probabilities; (2) \textit{Temperature scaling} \citep{kull2019beyond}, which scales the model's output using a learned parameter, whose efficacy for regression models depends on the output's monotonicity in relation to confidence; (3) \textit{Histogram binning} \citep{zadrozny2001obtaining}, a method partitioning predicted values into bins, calibrating each independently according to observed frequencies, yet might lack flexibility for diverse prediction intervals; (4) \textit{Platt scaling} \citep{kuleshov2018accurate}, which applies a scaling transformation to the predicted values with the function derived from minimizing observed and predicted value discrepancies, providing linear adaptability but potentially inadequate for complex uncertainty patterns; (5) \textit{Quantile regression} \citep{chung2021beyond}, details in Section \ref{sec:qr}.
% \begin{itemize}
%     \item \noindent\textit{Isotonic regression} \citep{niculescu2005predicting}, which ensures non-decreasing predictive probabilities, assuming higher model accuracy with increased predicted probabilities;

%     \item \noindent\textit{Temperature scaling} \citep{kull2019beyond}, which scales the model's output using a learned parameter, whose efficacy for regression models depends on the output's monotonicity in relation to confidence;

%     \item \noindent\textit{Histogram binning} \citep{zadrozny2001obtaining}, a method partitioning predicted values into bins, calibrating each independently according to observed frequencies, yet might lack flexibility for diverse prediction intervals;

%     \item \noindent\textit{Platt scaling} \citep{kuleshov2018accurate}, which applies a scaling transformation to the predicted values with the function derived from minimizing observed and predicted value discrepancies, providing linear adaptability but potentially inadequate for complex uncertainty patterns;
%     \item \noindent\textit{Quantile regression} \citep{chung2021beyond}, aforementioned.
% \end{itemize}


% \noindent\textit{Quantile regression} \citep{chung2021beyond}, an approach that minimizes the absolute difference between observed and predicted values using an asymmetrically weighted objective function, rendering it appropriate for calibration of asymmetric distributions.




% \begin{figure*}[!t]
%     \centering    
%     \subfigure[Calibration result using full data]{\includegraphics[scale=0.95]{figs/calibration_crime_1h.pdf}\label{fig:ccr1h_full}}
%     \subfigure[Calibration result using sparsity entries only]{\includegraphics[scale=0.95]{figs/calibration_crime_zero_1h.pdf}\label{fig:ccr1h_zero}}
%     \caption{Different calibration methods comparison on different components of STGCN-NB model outputs on data CCR\_1h.}
%     \label{fig:ccr1h}
% \end{figure*}



\subsection{Calibration Results Comparison}

% In our study, we applied an array of calibration methodologies to models trained using 60\% of the dataset. These models output parameters $\mu$ and $\alpha$, which in turn yield mean value predictions and PIs. We then recalibrated these models using an independent validation set, adjusting parameters for techniques such as temperature scaling, isotonic regression, Platt scaling, and quantile regression. A novel facet of our approach was the introduction of sparsity-aware calibration, where predictions with mean values below $0.5$ were identified as zero. This approach allowed for the calibration of models tailored specifically for this subset of data. For computing ENCE on ground-truth zero values, we used genuinely zero data instances, thereby ensuring precise uncertainty calibration measurement.

The calibration performance of the initial models and our proposed calibration methods is presented in Table \ref{tab:ce_full}. The ``zero-only targets'' refers to computing the ENCE exclusively on the true target values that are zeroes. Table \ref{tab:ce_full} demonstrates superior performance within each dataset with bold type and underlines the second-best results. Our findings reveal that the SAUC method typically outperforms other models, though it might fall short in aggregated cases, such as those with a 1-week resolution. Interestingly, the SAUC method achieved approximately a 23\% reduction in ENCE compared to the second-best model when using full observations and also about a 20\% reduction in sparsity entries. The separation of zero and non-zero data during calibration proved particularly beneficial, effectively addressing the issues of heteroscedasticity and zero inflation, commonly found in real-world datasets. However, we observed that calibration methods sometimes do not improve or even worsen calibration errors, mainly due to overfitting on the calibration set, which is particularly evident in temperature scaling and isotonic regression methods. 

On a general note, histogram binning and isotonic regression showed similar calibration results among baseline models as Equation \ref{eq:cdf} is non-decreasing, which makes the two methods easier to fit. Temperature scaling provides better calibration results in coarse temporal resolution scenarios and Platt scaling excels in sparse cases. QR consistently ranks as the second-best model in many cases, and our SAUC method has a close performance as QR in aggregated non-sparse cases but excels notably in sparse cases.


\subsection{Reliability Diagram Evaluation}

Utilizing Equations~\ref{eq:define_calib} and~\ref{eq:ence}, we refine the conventional reliability diagram to evaluate the calibration efficacy of a model \citep{kull2019beyond}. This involves partitioning predictions into bins based on $\mathcal{I}$, after which we compute the RMSE and MPIW employing the calibrated $\mu^*$ and $|\mathcal{I}^*|$ for each respective bin.

Figure \ref{fig:ccr8h} presents a comparative reliability diagram of STGCN-NB outputs prior to calibration, alongside Isotonic regression, Platt scaling, and our SAUC method, each applied to different segments of the CCR\_8h dataset. We selectively feature representative non-parametric and parametric baseline calibration approaches based on their performance. The diagonal dashed line symbolizes the calibration ideal: a closer alignment to this line indicates superior calibration.

\begin{figure*}[!ht]
    \centering    
    \subfigure[Full observations, CCR\_8h]{\includegraphics[scale=1]{figs/calibration_crime.pdf}\label{fig:ccr8h_full}}
    \subfigure[Zero-only targets, CCR\_8h]{\includegraphics[scale=1]{figs/calibration_crime_zero.pdf}\label{fig:ccr8h_zero}}
    \subfigure[Full observations, CCR\_1h]{\includegraphics[scale=1]{figs/calibration_crime_1h.pdf}\label{fig:ccr1h_full}}
    \subfigure[Zero-only targets, CCR\_1h]{\includegraphics[scale=1]{figs/calibration_crime_zero_1h.pdf}\label{fig:ccr1h_zero}}    \vspace{-0.8em}
    \caption{Reliability diagrams of different calibration methods applied to STGCN-NB outputs on different components of CCR\_8h and CCR\_1h data. Results closer to the diagonal dashed line are considered better.}
    \label{fig:ccr8h}
\end{figure*}

A closer examination of Figure \ref{fig:ccr8h_full} reveals that both baseline models and our SAUC technique adeptly calibrate the model outputs across all observations. Yet, focusing solely on the reliability diagram of our calibrated outputs for ground-truth zero values, as depicted in Figure \ref{fig:ccr8h_zero}, there is a noticeable deviation from the ideal line. Conversely, our SAUC approach demonstrates commendable alignment with the ideal when authentic data are zeros. This observation remains consistent for the CCR\_1h dataset, as seen in Figures \ref{fig:ccr1h_full} and \ref{fig:ccr1h_zero}. By contrasting Figures \ref{fig:ccr8h_full} and \ref{fig:ccr1h_full}, it becomes evident that the calibration performance diminishes in scenarios with finer resolutions. Nevertheless, our SAUC technique retains commendable efficacy, particularly when predicting zero entries, attributed to our distinctive calibration approach coupled with QR's adeptness at managing heteroscedasticity, especially when predictions on zeros exhibit considerable variability. Contemporary probabilistic spatiotemporal prediction models predominantly prioritize refining MPIWs for enhanced accuracy, often unintentionally neglecting practical safety considerations. Our calibration strategy offers outputs with reinforced reliability.


\section{Deployment}
\subsection{Risk Evaluation}
Funded by the U.S. Department of Energy (DoE) and the Chicago Transit Authority (CTA), our research supports the Vision Zero projects that eliminate traffic death by reliable risk evaluation \citep{belin2012vision,johansson2009vision}. We evaluate the use of SAUC outputs in accurately quantifying the uncertainty and potential risks of traffic crashes, thereby enhancing the downstream risk mitigation strategies. We introduce Risk Score (RS), an enhancement of the traditional metric defined as the product of \textit{event probability} and \textit{potential loss magnitude} \citep{ng2002algorithm,vose2008risk}:

\begin{equation}
    RS = \hat{\mu} \times |\hat{\mathcal{I}}|.
\end{equation}

This metric integrates anticipated risk ($\hat{\mu}$) and prediction uncertainty ($|\hat{\mathcal{I}}|$), attributing higher RS to regions with both high incident frequency and uncertainty. This RS metric assigns higher risk to predictions, characterized by large predicted mean values and high uncertainty.


\begin{figure}[!ht]
    \centering
    \subfigure[Avg. number of crashes]{\includegraphics[width=0.23\textwidth]{figs/case_study_expected.pdf}\label{fig:case_study_expect}}   \hfill 
    \subfigure[RS distribution using prediction before calibration]{\includegraphics[width=0.23\textwidth]{figs/RS_before_avg.pdf}\label{fig:case_study_before}}
    
    \subfigure[RS distribution using calibrated prediction via Platt scaling]{\includegraphics[width=0.23\textwidth]{figs/RS_calib_baseline.pdf}\label{fig:case_study_baseline}} \hfill
    \subfigure[RS distribution using using calibrated prediction via SAUC]{\includegraphics[width=0.23\textwidth]{figs/RS_calib_avg.pdf}\label{fig:case_study_calib}}
    \vspace{-0.8em}
    \caption{Traffic crash accident distributions and calibration using CTC\_8h data. All the data are averaged over the temporal dimension.}
    \label{fig:case_study}
\end{figure}

Using the CTC\_8h dataset and outputs from STGCN-NB, we demonstrate the importance of SAUC for evaluating the risks of traffic accidents. Figure \ref{fig:case_study} compares the average number of crashes and average RS values over time for each region, pre and post-calibration. Prior to calibration, as depicted in Figure \ref{fig:case_study_before}, the RS in regions, especially Chicago's northern and southern sectors, did not provide actionable insights, given their frequent traffic incidents reported by Figure \ref{fig:case_study_expect}. This is due to the tight PIs from pre-calibration model outputs lower the RS. As shown in Figure \ref{fig:case_study_baseline}, RS distribution from Platt scaling calibrated predictions could highlight certain risky areas, but still miss the major crash regions in southern Chicago. In contrast, SAUC-derived predictions, as seen in Figure \ref{fig:case_study_calib}, unveil coherent spatial distribution patterns highly consistent with Figure \ref{fig:case_study_expect}, demonstrating the effectiveness for urban safety monitoring.

Rather than just yielding exact numerical predictions with tight confidence intervals, it is imperative that models convey equivalent severity levels when integrating uncertainty. Such an approach ensures reliable outputs in crime and accident predictions. Notably, the reliable estimation of zero or non-zero incident counts is pivotal in risk management. Existing probabilistic prediction studies focus on exact values and restricted confidence intervals, sometimes neglecting the data variability, especially around zero incidences.

% \vspace{-2mm}
\subsection{Deployment Milestones and Obstacles} 
% Funded by the U.S. DoE and CTA, our project applies deep reinforcement learning (DRL) to mitigate bus bunching in Chicago. A critical element is developing a robust demand prediction model for reinforcement learning and optimization.

% \textcolor{red}{Maybe we can remove the DRL description since we did not focus on it in this paper. We can mention} 

% In collaboration with CTA, we have integrated our SAUC model into the bus decision-making (scheduling) system.

\noindent \textit{Milestones Reached:} In collaboration with CTA, we have integrated existing online prediction models and designed a robust demand-driven bus scheduling system. After presenting our design to the transit agency and incorporating their feedback, we are now implementing it with the data platform of CTA to demonstrate its efficacy. The next phase will involve small-scale field online testing.

% \textit{Deployment Obstacles:} Our system's deployment faces challenges including response speed limitations and potential mis-specifications in intricate travel demand scenarios. The non-interpretability of current spatiotemporal GNNs complicates the decision-making process, a concern addressable by explainable deep learning techniques \citep{ras2022explainable}. Furthermore, government staff's difficulty to grasp and implement our methods highlights the need for user-friendly tools and extensive training. Additionally, data and model privacy issues limit our access for post-hoc calibration, restricting us from conducting local training and testing of comprehensive baseline models, thereby excluding these results from our analysis.

\textit{Deployment Obstacles:} The deployment of our system encounters technical challenges, such as response speed limitations and potential mis-specifications in complex travel demand scenarios. The non-interpretability of existing spatiotemporal GNNs complicates the decision-making process, which could be mitigated through explainable deep learning techniques \citep{ras2022explainable}. Additionally, the difficulty faced by government staff in understanding and applying our methods underscores the importance of developing user-friendly tools and providing comprehensive training. A notable practical obstacle is our reliance on accessing data and models from a platform for post-hoc calibration without the ability to train and test full baseline models locally, due to data and model privacy concerns, preventing the inclusion of these results in our analysis.

==> backup_KDD_sections/6.Conclusion.tex <==
\vspace{-1mm}
\section{Conclusion}
Existing spatiotemporal GNN models primarily predict deterministic values, which neglect the uncertainties inherent in data. Particularly, the high-resolution spatiotemporal data is largely sparse and exhibits asymmetric distributions, so it presents further challenges to quantify the uncertainty. To address this challenge, in this paper, we propose the SAUC method that calibrates uncertainties across both zero and non-zero values. By transforming GNN-based deterministic models to probabilistic ones, SAUC aligns prediction uncertainty with the zero-inflated nature of spatiotemporal datasets. We also design novel PI-based calibration metrics for sparse and asymmetric distributions. Empirical assessments on two real-world datasets demonstrate the efficacy of the SAUC method, with an approximate 20\% reduction in calibration errors for zero-only targets in sparse cases. SAUC not only complements existing GNN models but also can be employed for risk evaluation in sparse datasets where reliable prediction uncertainty is imperative due to inherent safety concerns. In collaboration with the CTA, we have developed and are currently testing a demand-driven bus control system in Chicago, addressing technical and usability challenges to prepare for future field testing and smoother implementation.

\vspace{-1mm}
\section*{Ackowledgement}
This material is based upon work supported by the U.S. Department of Energy’s Office of Energy Efficiency and Renewable Energy (EERE) under the Vehicle Technology Program Award Number DE-EE0009211.

==> backup_sections/1.Introduction.tex <==
\section{Introduction}

Spatiotemporal GNNs have been instrumental in leveraging spatiotemporal data for various applications, from weather forecasting to urban planning \citep{wu2021inductive, zhao2022multi,gao2023spatiotemporal}. However, most of the models are narrowly focused on deterministic predictions, which overlooks the inherent uncertainties associated with the spatiotemporal phenomena. For various safety-related tasks, such as traffic accident and crime prediction, it is crucial to quantify their uncertainty, thus proactively preventing such phenomena from happening. Despite its importance, uncertainty quantification (UQ) remains relatively understudied in the spatiotemporal context, which can lead to erroneous predictions with severe social consequences \citep{chung2021beyond,abdo2017uncertainty,rudin2019stop}.

\redfont{add the barplot/histogram of the pmf in Figure 1a. Just keep Figure 1a. Put Figure 1b to the appendix.}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/sparsity_transition_hist.pdf}
    \caption{\redfont{Modify accordingly}. Comparative visualization of log-transformed crime counts for different temporal resolutions in the Chicago traffic crash dataset: (a) The KDE plot demonstrates the asymmetric data distribution shape in fine resolutions. (b) The CDF plot illustrates emphasizing the asymmetry. Median values are marked by vertical dashed lines, and horizontal lines quantify the data below the median, where a value of 0.5 denotes symmetry. 'Sparsity' denotes the proportion of zero-count instances within each temporal resolution.}
    \label{fig:sparsity_transition}
\end{figure}

Recent research has addressed UQ in spatiotemporal modeling \citep{wang2023uncertainty,zhuang2022uncertainty,huang_uncertainty_2023}, but often fails to account for the sparsity and asymmetrical distribution present in detailed spatiotemporal data. This sparsity, marked by an abundance of zeros, becomes pronounced when working with high-resolution data. Thus, effectively managing aleatoric (data) uncertainty is crucial in these applications. As shown in Figure \ref{fig:sparsity_transition}, the KDE plot for traffic crash counts at varying temporal resolutions shows a distinct move toward greater asymmetry as data resolution increases—evidenced by the horizontal line values in the CDF plot gradually rising above 0.5. Such a trend highlights the sporadic nature of traffic incidents, indicating that predictive models must adeptly address sparse data to truly reflect and forecast the temporal patterns observed.

Prior spatiotemporal GNNs with basic UQ functionalities typically model data using Negative Binomial (NB) or Gaussian distributions for regression tasks, focusing on learning these distributions' parameters for spatiotemporal predictions \citep{jiang2023uncertainty,zhuang2022uncertainty,wang2023uncertainty}. However, such models often require longer training time due to the use of distribution likelihoods as loss functions. A key limitation is their inadequate evaluation of UQ reliability using robust calibration metrics. Research by \citep{zhuang2022uncertainty,wu2021quantifying,jiang2023uncertainty,gao2023spatiotemporal} often emphasizes high accuracy and narrow prediction intervals as indicators of effective UQ. This approach overlooks the crucial relationship between data variance and prediction intervals, which is vital for addressing aleatoric uncertainty. As highlighted by \citet{kuleshov2018accurate}, most deep learning models are not fully calibrated for high UQ quality, leaving a significant research gap to be filled.

This paper introduces a sparsity-aware uncertainty calibration (SAUC) method, calibrating model outputs to align with true data distributions, which can be adapted to any spatiotemporal GNN model. Inspired by the zero-inflated model, we partition zero and non-zero predictions and apply separate Quantile Regression (QR) models to ensure the discrepancy of prediction and true values lie within the PIs. This post-hoc approach, unlike uncertainty-aware spatiotemporal prediction models \citep{rahman_uncertainty-aware_2023}, offers flexibility in applying it to existing models without necessitating architectural or loss function changes or full model retraining. Consistent with prior studies on regression task calibration, we formulate a modified calibration metric tailored for PI-based calibration within asymmetric distributions. To investigate our model's generalizability, we adapt two prevalent spatiotemporal GNN models with negative binomial distributions to suit sparse settings without compromising prediction accuracy. After being tested on two real-world spatiotemporal datasets with different levels of sparsity, our SAUC demonstrates promising calibration results, thus assisting in reliable decision-making and risk assessment.
We summarize he main contributions of this paper in threefold:
\begin{itemize}
    \item We design a novel sparsity-aware uncertainty calibration (SAUC) method for predicting sparse spatiotemporal data, which is adaptive to existing GNN models and applicable to any probabilistic outputs.
    \item We focus on the calibration of asymmetric distributions, like the NB, using quantile regression. This approach deviates from conventional mean-variance UQ methods. Additionally, we have developed new calibration metrics based on prediction interval width.
    \item We conduct experiments on different real-world sparse datasets to demonstrate promising calibration results of our SAUC, especially for zero values. We observe a roughly \textbf{20\% reduction} in calibration errors relative to leading baseline models, underscoring its efficacy for safety-critical decision-making.
\end{itemize}


==> backup_sections/2.RelatedWork.tex <==
\section{Related Work}
% \subsection{DL in Spatiotemporal Prediction}
% \redfont{Existing work do not consider UQ first }

\subsection{Spatiotemporal Prediction}

% \subsection{UQ in Spatiotemporal Deep Learning}
% Spatiotemporal prediction leveraging deep learning and Graph Neural Networks (GNNs) has emerged as a powerful tool in machine learning, providing invaluable insights for diverse applications, including traffic forecasting, climate modeling, and urban planning. However, there's a significant research gap regarding Uncertainty Quantification (UQ) in these models. The lack of focus on UQ leads to overlooked uncertainties in predictions, compromising their reliability.

% UQ in spatiotemporal prediction plays a crucial role in measuring the confidence and reliability of the prediction results. Two principal methodologies have been employed for this purpose, namely, the Bayesian and Frequentist approaches \citep{wang2023uncertainty, zhuang2022uncertainty,zhao2022multi}. The Bayesian paradigm, grounded in parameter inference techniques such as Laplace approximation, Markov Chain Monte Carlo (MCMC), and Variational Inference (VI), offers critical insights. However, it is often hampered by computational complexities and inaccuracies arising from approximation \citep{wu2021bayesian,qian2022uncertainty,wu2021quantifying,gawlikowski2021survey}.

% On the contrary, the Frequentist approach leverages Mean-Variance Estimation (MVE), leading to computational efficiency and flexibility in model construction \citep{wang2023uncertainty}. This approach encompasses both parametric and non-parametric methods, with the former incorporating probabilistic layers for UQ, and the latter primarily focusing on the establishment of prediction intervals. It is worth noting that while these methods have demonstrated utility, non-parametric approaches heavily depend on data abundance, whereas parametric methods are predominantly reliant on predefined data distributions \citep{wu2023adaptive,gawlikowski2021survey}.

% While parametric methods are generally preferred due to computational efficiency and adaptability, their application to sparse and event-centric spatiotemporal data is markedly limited \citep{jiang2023uncertainty}. \citet{zhuang2022uncertainty} and \citet{gao2023uncertainty} have introduced zero-inflated distributions in conjunction with spatiotemporal neural networks. This amalgamation was used to manage the prevalent zero instances and non-normal distribution found in sparse travel demand data. However, they confronted practical challenges when zero values were excessively extreme, especially in non-time series scenarios such as event-based risk situations, including traffic accidents and urban crime prediction. In these scenarios, the accuracy of predicting zeroes or non-zeroes significantly impacts the reliability and robustness of system design and monitoring. Consequently, the quantification and calibration of uncertainty within the sparsity component of spatiotemporal data is not only vital but also currently under-explored.


Spatiotemporal prediction through deep learning offers a powerful tool for various applications. Among them, GNNs have become prevalent in recent years \citep{wu2021inductive,zhao2022multi,yu2017spatio,wu2019graph}. Most existing models focus on predicting the deterministic values without considering the associated uncertainty, which leaves a noticeable research gap concerning UQ. Such a limitation impacts the reliability of predictions, as the unaccounted uncertainty can lead to deviations from the true data variance.

Bayesian and Frequentist approaches are the two main existing methods for spatiotemporal UQ \citep{wang2023uncertainty,zhou2021stuanet}. While the Bayesian approach offers profound insights through techniques like Laplace approximation \citep{wu2021bayesian}, Markov Chain Monte Carlo \citep{pearce2018high}, and Variational Inference \citep{khosravi2010lower}, it suffers from computational complexities and approximation inaccuracies. In contrast, the Frequentist approach exploits Mean-Variance Estimation for computational efficiency and model flexibility, accommodating both parametric and non-parametric methods \citep{wang2023uncertainty}. However, the application of these methods to sparse data is challenged by data dependencies and distribution constraints \citep{wu2023adaptive,gawlikowski2021survey}. For example, sparse data frequently deviate from models' mean-variance assumptions, favoring NB distributions over Gaussian, and traditional metrics like mean squared errors can be skewed by sparse datasets' non-zero values.
%sparse data often do not fit common models' mean-variance assumptions,

The use of zero-inflated distributions with spatiotemporal neural networks has been introduced to handle zero instances and non-normal distribution in sparse data \citep{zhuang2022uncertainty}. However, this approach has limitations in extreme scenarios and non-time-series contexts, impacting predictive accuracy and system robustness \citep{wang2023uncertainty,10.1145/3583780.3615215,qian2023uncertainty}. Therefore, the urgent need to quantify and calibrate uncertainty in the sparse component of spatiotemporal data is evident, yet remains largely unexplored.

\subsection{Uncertainty Calibration}
Although relatively understudied in the spatiotemporal context, UQ has been examined by many machine learning studies. Among all the UQ approaches, calibration is a post-hoc method that aims to match the predictive probabilities of a model with the true probability of outcomes, developing robust mechanisms for uncertainty validation \citep{nixon2019measuring}.

A wealth of techniques has been developed to calibrate pre-trained classifiers, mitigating the absence of inherent calibration in many uncertainty estimators \citep{kumar2019verified,gruber2022better,shen2023post}. Calibration for regression tasks, however, has received less attention \citep{thiagarajan2020building,kuleshov2018accurate}. Post-hoc calibration methods for classifications, such as temperature scaling, Platt scaling, and isotonic regression, have successfully been adapted for regression \citep{kull2019beyond}. \citet{chung2021beyond} further demonstrated quantile regression-based calibration methods and their extensions. These post-hoc methods offer greater flexibility and wider applicability to various probabilistic outputs compared to in-training methods, without necessitating model retraining \citep{rahman_uncertainty-aware_2023,huang_uncertainty_2023}.

In sparse spatiotemporal data contexts, where accurate model outputs are important for applications like traffic accident forecasting and crime prediction \citep{zhao2022multi}, the significance of uncertainty calibration is often overlooked. Traditional calibration methods focus on symmetric distributions like Gaussian, but sparse datasets commonly align with asymmetric NB distributions. Given the zero-inflated characteristics of such data, it is essential to discern confidence for zero and non-zero segments due to their varied implications. In response, we propose the SAUC method to manage asymmetric distributions and ensure empirical variances of true targets align with estimated PIs \citep{thiagarajan2020building}.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width= 0.8\textwidth ]{figs/models.pdf}
    \caption{ \redfont{Change the linear layer into prediction layer. Echo in the modification parts. The likelihood one line and two branches. Remove H from the figure.} Framework of models and experiments. We modify existing spatiotemporal GNNs into probabilistic ones with NB distribution parameters as the outputs. Sparsity-aware uncertainty calibration are then conducted to obtain the quantile regression results and calibrated confidence interval for forecasting. These two steps are easy and practical to generalize all existing spatiotemporal GNNs. }
    \label{fig:model}
\end{figure*}

==> backup_sections/3.Preliminary.tex <==
\section{Problem Formulation}
% In this section, we introduce mathematical notations and problem formulations for the spatiotemporal prediction task and the associated uncertainty calibration process.

% Let $\mathcal{G} = (V,E,A)$ where $V$ represents the set of nodes (locations), $E$ the edge set, and $A\in \mathbb{R}^{|V|\times|V|}$ the adjacency matrix describing the relationship between nodes. Denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|V| \times t}$ where $t$ is the number of time steps. For simplicity, 

% The objective is to predict the value $y_{1:|V|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|V|,1:t}$. A predictive GNN model $f_{\theta}$, parametrized by $\theta$, generates the output $\hat{y}_{1:|V|,t:t+k} = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G})$. 

% With the emerging interest in probabilistic GNNs for discrete spatiotemporal predictions, the aim extends beyond mere predictions, seeking to capture the associated uncertainty, calling it UQ \citep{zhuang2022uncertainty,jiang2023uncertainty,wang2023uncertainty}. In our context, we assume each element $\hat{y}_{i,j}$ of model output $\hat{y}_{1:|V|,t:t+k}$ follows NB distribution characterized by shape parameter $\mu_{i,j}$ and dispersion parameter $\alpha_{i,j}$. The GNN model, in this probabilistic context, is then reformulated as follows:
% \begin{equation}
%     (\hat{\mu}_{1:|V|,t:t+k},\hat{\alpha}_{1:|V|,t:t+k}) = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G}).
% \end{equation}
% Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as delineated in Equation \ref{eq:modify_loss}.


\subsection{Spatiotemporal GNNs for Prediction} 
\noindent Let $\mathcal{G} = (\mathcal{V},\mathcal{E},\mathbf{A})$ where $\mathcal{V}$ represents the set of nodes (locations), $\mathcal{E}$ the edge set, and $\mathbf{A}\in \mathbb{R}^{|\mathcal{V}|\times|\mathcal{V}|}$ the adjacency matrix describing the relationship between nodes. By default, we differentiate script and italic alphabets for sets and data points. We denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|\mathcal{V}| \times t}$ where $t$ is the number of time steps. The objective is to predict the target value $\mathcal{Y}_{1:|\mathcal{V}|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|\mathcal{V}|,1:t}$. The full dataset is partitioned by timesteps into training, calibration (i.e., validation), and testing sets. The three data partitions are denoted as $\mathcal{X}_{T}$, $\mathcal{X}_{S}$, and $\mathcal{X}_{U}$, respectively. For example, the training set $\mathcal{X}_{1:|\mathcal{V}|,1:t}$ is denoted as $\mathcal{X}_{T}$. The associated target values are represented as $\mathcal{Y}_{T}$, $\mathcal{Y}_{S}$,  and $\mathcal{Y}_{U}$, with subscripts indicating the corresponding sets.

The objective of the spatiotemporal GNN models is to design model $f_{\theta}$, parametrized by $\theta$, which yields:
\begin{equation}
    \hat{\mathcal{Y}}_d = f_{\theta}(\mathcal{X}_d; \mathcal{G}), \forall\ d \in \{ T,S,U \},
    \label{eq:GNN}
\end{equation}
where $\hat{\mathcal{Y}}_d$ is the predicted target value, and the subscript represents the corresponding data set. Note that $\theta$ is fixed once $f_{\theta}$ is trained on set $T$.

With emerging interests in quantifying the data and model uncertainty of spatiotemporal GNNs, researchers shift towards designing probabilistic GNNs to predict not only mean values but also PIs \citep{zhuang2022uncertainty, jiang2023uncertainty, wang2023uncertainty}. Previous probabilistic spatiotemporal GNN studies often assume $\mathcal{X}$ and $\mathcal{Y}$ encompassing independent and identically distributed Gaussian random variables $X_i$ and $Y_i$, which are assumed as NB distributions to accommodate the sparse data in this study. The NB distribution of each predicted data point is characterized by shape parameter $\mu$ and dispersion parameter $\alpha$. Previous work has applied linear layers after spatiotemporal GNNs to study the parameter sets of the predicted data points \citep{zhuang2022uncertainty,jiang2023uncertainty}. The set of predicted $\mu$ and $\alpha$ corresponding to all elements of $\mathcal{Y}$ are denoted as $\hat{M}$ and $\hat{H}$. Therefore, Equation \ref{eq:GNN} can be rewritten in the format of NB distribution based probabilistic spatiotemporal GNNs as:
\begin{equation}
    (\hat{M}_d,\hat{H}_d) = f_{\theta} (\mathcal{X}_d; \mathcal{G}), \forall d \in \{ T,S,U \}.
    \label{eq:PGNN}
\end{equation}
Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as delineated in Equation \ref{eq:modify_loss}.

\subsection{Prediction Interval Calibration}
Uncertainty calibration refines the outputs of predictive models, such as GNNs, to ensure that predicted distributions accurately reflect actual distributions. Traditionally, calibration methods presuppose that data follow a Gaussian distribution, characterized by mean and variance parameters. However, for sparse datasets, the NB distribution, which typically exhibits right skewness, is a more appropriate choice \citep{zhuang2022uncertainty}. Unlike the Gaussian distribution, where prediction interval widths are directly calculable from variance and z-scores, the NB distribution does not offer a simple expression for prediction intervals based on its parameters. Therefore, our calibration method concentrates on aligning prediction intervals with data variance rather than modifying the NB distribution's parameters. This strategy builds upon and expands earlier research that prioritizes variance considerations.

The spatiotemporal prediction models generate outputs the sets of location and shape parameters $\hat{M}_d,\hat{H}_d, \forall d \in \{ T, S, U\}$, in which $\hat{\mu}_i \in \hat{M}_d$ is the mean value of the predicted distribution. We then construct the prediction intervals of the NB distributions as $\hat{\mathcal{I}}_i = [\hat{l}_i,\hat{u}_i]$ with $\hat{l}_i$ and $\hat{u}_i$ denoting the 5th- and 95th-percentiles, respectively. Notably, our discussion limits the prediction intervals to the 5\% and 95\% range. Based on \citet{kuleshov2018accurate}, our target is to ensure a prediction model $f_{\theta}$ to be calibrated, i.e.,
\begin{equation}
    \frac{ \sum_{i=1}^{|U|} \mathbb{I}\{ y_{i} \leq \hat{F}_{i}^{-1}(p) \} }{|U|} \xrightarrow{|U| \rightarrow \infty} p,\  \forall p \in \{0.05, 0.95\},
    \label{eq:pi_calib}
% |V|\times k \rightarrow \infty
\end{equation}
where $p$ stands for the targeting probability values, $\mathbb{I}$ denotes the indicator function, and $\hat{F}_{i}(\cdot)$ is the CDF of the NB distributions parameterized by $\hat{\mu}_{i}$ and $\hat{\alpha}_{i}$. The primary goal is to ensure that, as the dataset size increases, the predicted CDF converges to the true one. Such an alignment is congruent with quantile definitions, suggesting, for instance, that 95\% of the genuine data should fall beneath the 95\% percentile. Rather than striving for a perfect match across $\forall p \in [0,1]$, we mainly focus on calibrating the lower bound and upper bound.

% \subsection{}
Empirically, we leverage the calibration set $S$ to calibrate the uncertainty in data. The empirical CDF for a given value $p \in \hat{F}_i (y_i)$ is computed \citep{kuleshov2018accurate,levi2022evaluating}:
\begin{equation}
    \hat{\mathcal{P}}(p) = \frac{ |\{ y_{i} | \hat{F}_i(y_i) \leq p, i = 1, \dots, |S| \} | }{|S|}.
    \label{eq:cdf}
\end{equation}
The calibration process entails mapping a calibration function $\mathcal{C}$, such as isotonic regression or Platt scaling, to the point set $\{ (p,\hat{\mathcal{P}}(p)) \}_{i=1}^{|S|} $. Consequently, the composition $\mathcal{C} \circ \hat{F}$ ensures that $\hat{\mathcal{P}}(p) = p$ within the calibration dataset. This composition can then be applied to the test set to enhance the reliability of predictions.



==> backup_sections/4.Methodology.tex <==
% \section{Methodology}
% In this section, we introduce mathematical notations, the general calibration process, and our proposed SAUC method. We first define the spatiotemporal prediction problem and then introduce the uncertainty calibration problem.


% % Let $\mathcal{G} = (V,E,A)$ where $V$ represents the set of nodes (locations), $E$ the edge set, and $A\in \mathbb{R}^{|V|\times|V|}$ the adjacency matrix describing the relationship between nodes. Denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|V| \times t}$ where $t$ is the number of time steps. For simplicity, 

% % The objective is to predict the value $y_{1:|V|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|V|,1:t}$. A predictive GNN model $f_{\theta}$, parametrized by $\theta$, generates the output $\hat{y}_{1:|V|,t:t+k} = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G})$. 

% % With the emerging interest in probabilistic GNNs for discrete spatiotemporal predictions, the aim extends beyond mere predictions, seeking to capture the associated uncertainty, calling it UQ \citep{zhuang2022uncertainty,jiang2023uncertainty,wang2023uncertainty}. In our context, we assume each element $\hat{y}_{i,j}$ of model output $\hat{y}_{1:|V|,t:t+k}$ follows NB distribution characterized by shape parameter $\mu_{i,j}$ and dispersion parameter $\alpha_{i,j}$. The GNN model, in this probabilistic context, is then reformulated as follows:
% % \begin{equation}
% %     (\hat{\mu}_{1:|V|,t:t+k},\hat{\alpha}_{1:|V|,t:t+k}) = f_{\theta} (\mathcal{X}_{1:|V|,1:t}; \mathcal{G}).
% % \end{equation}
% % Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as delineated in Equation \ref{eq:modify_loss}.



% \noindent\textbf{Spatiotemporal Prediction using GNNs.} Let $\mathcal{G} = (\mathcal{V},\mathcal{E},\mathbf{A})$ where $\mathcal{V}$ represents the set of nodes (locations), $\mathcal{E}$ the edge set, and $\mathbf{A}\in \mathbb{R}^{|\mathcal{V}|\times|\mathcal{V}|}$ the adjacency matrix describing the relationship between nodes. Denote the spatiotemporal dataset $\mathcal{X} \in \mathbb{R}^{|\mathcal{V}| \times t}$ where $t$ is the number of time steps. The objective is to predict the target value $\mathcal{Y}_{1:|\mathcal{V}|,t:t+k}$ of future $k$ time steps given all the past data up to time $t$, which is $\mathcal{X}_{1:|\mathcal{V}|,1:t}$. For the sake of clarity, and considering all nodes are incorporated into the analysis, we partition the dataset by timesteps into training, recalibration (i.e., validation), and testing sets. These datasets partitions are denoted by $\mathcal{X}_{T}$, $\mathcal{X}_{S}$,  and $\mathcal{X}_{U}$, respectively. For example, $\mathcal{X}_{1:|\mathcal{V}|,1:t}$ is denoted as $\mathcal{X}_{T}$. The associated target values are represented as $\mathcal{Y}_{T}$, $\mathcal{Y}_{S}$,  and $\mathcal{Y}_{U}$, with subscripts indicating the corresponding sets.

% The objective of the spatiotemporal GNN models is to design model $f_{\theta}$, parametrized by $\theta$, which yields:
% \begin{equation}
%     \hat{\mathcal{Y}}_d = f_{\theta}(\mathcal{X}_d; \mathcal{G}), \forall\ d \in \{ T,S,U \},
%     \label{eq:GNN}
% \end{equation}
% where $\hat{\mathcal{Y}}_d$ is the predicted target value, and the subscript represents the corresponding data set. Note that $\theta$ is fixed once $f_{\theta}$ is trained on set $T$.

% With the emerging interest in quantifying the data and model uncertainty of spatiotemporal GNNs, there is a shift towards utilizing probabilistic GNNs that predict not only mean values but also PIs \citep{zhuang2022uncertainty,jiang2023uncertainty,wang2023uncertainty}. In previous probabilistic spatiotemporal GNN studies, $\mathcal{X}$ and $\mathcal{Y}$ are assumed to consist of independent and identically distributed random variables $X$ and $Y$. In our study, $X$ and $Y$ are assumed to follow NB distributions when predicting discrete data. The NB distribution of each predicted data point is characterized by shape parameter $\mu$ and dispersion parameter $\alpha$. The set of predicted $\mu$ and $\alpha$ corresponding to all elements of $\mathcal{Y}$ are denoted as $\hat{M}$ and $\hat{H}$. Therefore, Equation \ref{eq:GNN} can be rewritten as:
% \begin{equation}
%     (\hat{M}_d,\hat{H}_d) = f_{\theta} (\mathcal{X}_d; \mathcal{G}), \forall d \in \{ T,S,U \}.
%     \label{eq:PGNN}
% \end{equation}
% Subsequently, the objective function is adjusted to incorporate the relevant log-likelihood, as delineated in Equation \ref{eq:modify_loss}.

% \subsection{Problem Formulation}
% Uncertainty calibration aims to refine the outputs of prediction models (e.g., GNNs) such that the predicted distributions align with the true distributions. Traditional calibration models generally assume Gaussian distributions, which only involve the mean and variance parameters due to their intrinsic relationships with output variances, like the two-sigma associations. However, when dealing with discrete and sparse data, adopting alternative distributions such as the NB distribution is more suitable due to their asymmetric nature. Thus, our calibration methodology gives prominence to the prediction interval, serving as a natural extension of previous variance-oriented studies.

% From the spatiotemporal prediction model, with the outputs $\hat{M}_d,\hat{H}_d, \forall d \in \{ T, S, U\}$, we recognize $\hat{\mu}_i \in \hat{M}_d$ as the mean value of the predicted distribution of an individual future data point. We then use the 5\% to 95\% confidence interval of the output NB distributions as the prediction intervals $\hat{\mathcal{I}}_i = [\hat{l}_i,\hat{u}_i]$ with $\hat{l}_i$ and $\hat{u}_i$ denoting the lower and upper bounds, respectively. Notably, our discussion limits the prediction intervals to the 5\% and 95\% range. Based on \citet{kuleshov2018accurate}, our target is to ensure a prediction model $f_{\theta}$ to be calibrated, i.e.,
% \begin{equation}
%     \frac{ \sum_{i=1}^{|U|} \mathbb{I}\{ y_{i} \leq \hat{F}_{i}^{-1}(p) \} }{|U|} \xrightarrow{|U| \rightarrow \infty} p,\  \forall p \in \{.05, .95\},
%     \label{eq:pi_calib}
% % |V|\times k \rightarrow \infty
% \end{equation}
% where $p$ stands for the confidence level, $\mathbb{I}$ denotes the indicator function, and $\hat{F}_{i}(\cdot)$ is the cumulative density function (CDF) of the NB distributions steered by $\hat{\mu}_{i}$ and $\hat{\alpha}_{i}$. The primary goal is to ensure that, as the dataset size increases, the predicted CDF converges to the true one. Such an alignment is congruent with quantile definitions, suggesting, for instance, that 95\% of the genuine data should fall beneath the 95\% percentile. Rather than striving for a perfect match across $\forall p \in [0,1]$, we mainly focus on calibrating the lower bound and upper bound, mirroring earlier calibration endeavors centered around mean and variance.

% \subsection{Prediction-interval Based Calibration}
% For recalibrating the uncertainty inherent in our prediction model, we leverage the model's output for the recalibration set $S$. The empirical CDF for a given predicted CDF value $p \in \hat{F}_i (y_i)$  is then computed \citep{kuleshov2018accurate,levi2022evaluating}:
% \begin{equation}
%     \hat{\mathcal{P}}(p) = \frac{ |\{ y_{i} | \hat{F}_i(y_i) \leq p, i = 1, \dots, |S| \} | }{|S|}.
%     \label{eq:cdf}
% \end{equation}
% The calibration process entails mapping a calibration function $\mathcal{C}$, such as isotonic regression or Platt scaling, to the point set $\{ (p,\hat{\mathcal{P}}(p)) \}_{i=1}^{|S|} $. Consequently, the composition $\mathcal{C} \circ \hat{F}$ ensures that $\hat{\mathcal{P}}(p) = p$ within the recalibration dataset. This composition can then be extended to the prediction outputs on the test set for enhanced reliability.

\section{Sparsity-Aware Uncertainty Calibration}
% Equation \ref{eq:cdf} pertains to CDF and quantiles, harmonizing with the objectives of QR. In the following, we delineate the fundamentals of QR, introduce our SAUC method rooted in QR, and outline metrics designed to gauge calibration discrepancies with respect to mean and PI predictions.
\subsection{QR for Uncertainty Calibration} 
%QR excels in modeling the conditional quantiles of a response variable, elevating its significance for uncertainty calibration. 
Unlike traditional regression techniques that target the conditional mean, QR predicts specific quantiles, which are essential for calibrating PIs. Given $\hat{M}_S$ and $\mathcal{Y}_S$ from the calibration set $S$, the linear QR model can be expressed as:
\begin{equation}
    Q_{\mathcal{Y}_S | \hat{M}_S }(p) = \hat{M}_S^T \beta(p),
    \label{eq:QR}
\end{equation}
where $\beta(p)$ signifies the coefficient associated with quantile $p$. The goal here is to minimize the Pinball loss \citep{chung2021beyond}, which is defined as: 

\begin{equation}
L_{\text{pinball}}(y, \hat{y}, p) =
\begin{cases}
(p-1) \cdot (y - \hat{y}), & \text{if } y < \hat{y} \\
p \cdot (y - \hat{y}), & \text{if } y \geq \hat{y}
\end{cases}.
\end{equation}
In our context, we focus on the cases of $p=5\%$ and 95\%, and thus the quantile regressions output calibrated PIs correspond to $[Q(0.05),Q(0.95)]$.

QR is adept at handling sparse datasets, addressing heteroscedasticity and capturing non-linear relationships. Sparsity can introduce heteroscedasticity, where error variance differs across observations. Without assuming constant variance, QR manages datasets with variance fluctuations, often arising from zeros. Moreover, when combined with basis expansion techniques, QR extends its capability to capture intricate patterns across quantiles, making it well-suited for areas where zero outcomes are prevalent.

\subsection{SAUC Method}
Our SAUC method is a two-step post-hoc calibration tailored for sparse data, as detailed in Figure \ref{fig:model}. We trained the modified NB based probabilistic spatiotemporal GNNs's to obtain the model parameters $f_\theta$ (modifications detailed later). This training yields shape and dispersion parameters $\hat{M}_S,\hat{H}_S$ on the calibration set for uncertainty calibration. Drawing inspiration from zero-inflated models, predictions in the calibration set $S$ are bifurcated based on \textbf{indices}: $I_{Z} = \{\hat{M}_S < 0.5\}$ for prediction values nearing zero, and $I_{NZ} = \{\hat{M}_S \geq 0.5\}$ for non-zero predictions. The value of 0.5 is a natural dividing line for the rounding operations to determine if values are effectively zeroes. Following this partitioning, two QR models, $Q_Z$ and $Q_{NZ}$, are trained separately, calibrating quantiles $p = \{ .05, .95 \}$ to fine-tune the mean and PI predictions. The calibrated model is then applied to predict model outputs on the testing set. Pseudocode details for implementing the SAUC method are provided in Algorithm \ref{alg:sauc} and codes can be found in the anonymous Github repository \footnote{\url{https://github.com/AnonymousSAUC/SAUC}}.

The SAUC method focuses on calibrating PIs rather than modifying distribution parameters, aligning with the principles of previous post-hoc calibration methods like isotonic regression and Platt scaling \citep{niculescu2005predicting,kuleshov2018accurate}. These methods are designed to refine a model's outputs without directly altering internal parameters such as the parameters $\mu$ and $\alpha$ of NB distributions. This strategy ensures a distinct separation between modeling and calibration, enhancing flexibility and broad applicability. It avoids complicating the calibration process and potentially impacting the core modeling objectives. Additionally, post-hoc methods have demonstrated practical effectiveness and computational efficiency in improving the probabilistic accuracy of predictions, without necessitating retraining or modifications to the original model

\begin{algorithm}[t]
\caption{SAUC Method}
\begin{algorithmic}[1]
\REQUIRE $\hat{M}_S$, $\mathcal{Y}_S$, $N$, $\hat{M}_U$, $p\leftarrow \{ .05, .95 \}$
\STATE Define the bin thresholds $\mathcal{T}_S$ using percentiles of $\mathcal{Y}_S$.
\STATE Initialize $U^*$, $L^*$ in the same size as $\hat{M}_U$.
\FOR{each bin $i$ in $[1, N]$}
\STATE Extract indices $I$ of instances in bin $i$ based on $\mathcal{T}_S$.
\STATE Split $I$ to $I_{NZ}$ for $\hat{M}_S\geq 0.5$ and $I_Z$ for $\hat{M}_S<0.5$.
\FOR{each set $i$ in $\{I_{NZ}, I_Z\}$}
\FOR{each value $q$ in $p$}
\STATE Fit $Q(q)$ on $\hat{M}_S[i]$ and $\mathcal{Y}_S[i]$ based on Equation \ref{eq:QR} and obtain $\beta (q)$.
\ENDFOR
\STATE 
% $M^*[i]\leftarrow \hat{M}_U^T \beta(.5)$,
$L^*[i]\leftarrow \hat{M}_U^T \beta(.05)$, $U^*[i]\leftarrow \hat{M}_U^T \beta(.95)$
\ENDFOR
\ENDFOR
\STATE $\mathcal{I}^* \leftarrow [L^*, U^*] $.
\RETURN $\mathcal{I}^*$.
\end{algorithmic}
\label{alg:sauc}
\end{algorithm}

% In the proposed SAUC method, special emphasis is given to local calibrations, particularly addressing data sparsity. While \citet{song2019distribution} have highlighted that a quantile-calibrated regression model offering predictions with specific empirical moments (e.g. mean and variance) does not ensure that targets with identical predicted moments universally maintain the same true moments, this is largely because traditional approaches contemplate the issue on a broad scale, calibrating quantiles globally. However, by partitioning the data into zero and non-zero segments, our method is designed to obtain nuanced quantile calibrations for these distinct components, each bearing unique implications. The zero segment, potentially substantial in size, necessitates meticulous calibration due to its binary nature in practical scenarios. Conversely, for the non-zero section, it's vital that predicted quantiles genuinely represent the actual event quantiles, as research in this domain typically seeks to interpret relative risks or event severities.

\citet{song2019distribution} argued that quantile regressions might not retain true moments for the targets with similar predicted moments because of the global averaging effects. This limitation is addressed by our SAUC method because it creates local segments based on zero and non-zero values. The zero segment, potentially dominant, requires precision in calibration due to its binary implications in real-world applications. For the non-zero subset, the aim is to ensure that quantiles mirror actual event frequencies, resonating with the typical research focus on discerning relative risks or magnitudes of events. Notice that, even though our SAUC method is discussed based on Equation \ref{eq:PGNN} in GNN models, it can be generalized to any spatiotemporal prediction task.

\subsection{Calibration Metrics for Asymmetric Distributions}

While calibration errors are clearly established for classification tasks using Expected Calibration Error \citep{nixon2019measuring,gruber2022better,kumar2019verified}, the definition is much less studied in the regression context, where prediction errors and intervals supersede accuracy and confidence. Based on Equation~\ref{eq:pi_calib} and~\ref{eq:cdf}, we aim to calibrate the length of the prediction interval with the variance, i.e.,
\begin{equation}
    \small
    \big[\mathbb{E}[ (\hat{\mu}_i - Y_i)^2 | \hat{\mathcal{I}_i} = \mathcal{I}_i ]\big]^{1/2} = c|\mathcal{I}_i|, \ \forall i \in \{ 1, \dots, |U| \}.
    \label{eq:define_calib}
\end{equation}
Note that $\mathcal{I}_i= [F_i^{-1}(.05),F_i^{-1}(.95)]$ is the realization of the predicted 5\%-95\% confidence interval and $|\mathcal{I}_i|$ denotes its width. Calibrating the model's standard errors with the 90\% confidence interval width reveals a linear relationship with coefficient $c$, specifically for symmetric distribution like Gaussian. As an approximation, we continue to use the z-score of Gaussian distribution to compute the coefficient $c$. The width of 5\%-95\% confidence interval is roughly $2\times 1.645 = 3.29$ of distribution variance, inversely proportional to $c$. Empirical results, illustrated in Figure \ref{fig:find_c}, support a linear correlation between the ratio of the predicted interval $\hat{\mathcal{I}}$ and the variance of the distribution. In our experiments, this slope ranges from 0.3 to 0.4, aligning closely with our theoretical assumption. Consequently, this leads to a value of $c \approx \frac{1}{3.29} \approx 0.303$.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/find_c.pdf}
    \caption{Explore the linear correlation between MPIW and RMSE using different cases of the CCR data.}
    \label{fig:find_c}
\end{figure}

Therefore, we could diagnose the calibration performance by comparing value differences on both sides of the equation. Specifically, we partition the \textbf{indices} of test set samples into $N$ evenly sized bins based on sorted predicted PI width, denoted as $\{B_j\}_{j=1}^N$. In our study, we set $N=15$ by default. Each bin corresponds to a PI width which falls within the intervals: $[\min_{i\in B_j}\{ |\mathcal{I}_i| \}, \max_{i\in B_j}\{ |\mathcal{I}_i| \}]$. Note that the intervals are non-overlapping and their boundary values are increasing. Based on the discussion of \citet{levi2022evaluating} and Equation \ref{eq:define_calib}, for $j$-th bin, we define the Expected Normalized Calibration Error (ENCE) based on Root Mean Squared Error (RMSE) and Mean Prediction Interval Width (MPIW):
\begin{equation}
ENCE = \frac{1}{N} \sum_{j=1}^N \frac{|c \cdot MPIW(j) -  RMSE(j) |}{c \cdot MPIW(j)},
\label{eq:ence}
\end{equation}
where the $RMSE$ and $MPIW$ are defined as:
\begin{align}
    RMSE(j) &= \sqrt{ \frac{1}{|B_j|} \sum_{i\in B_j} (\hat{\mu}_i - y_i)^2 }\\
    MPIW(j) &= \frac{1}{|B_j|} \sum_{i \in B_j} |\hat{\mathcal{I}}_i|
\end{align}

This normalizes calibration errors across bins, sorted and divided by $c \cdot MPIW$, and is particularly beneficial when comparing different temporal resolutions and output magnitudes across datasets. The $c \cdot MPIW$ and observed $RMSE$ per bin should approximate equality in a calibrated forecaster.



==> backup_sections/5.Experiments.tex <==
\section{Experiments}


% \begin{table*}[!t]
%     \scriptsize
%     \centering    
%     \begin{tabularx}{\linewidth}{c*{7}{>{\centering\arraybackslash}X}@{\hspace{4pt}}c@{\hspace{4pt}}*{7}{>{\centering\arraybackslash}X}}
%     \toprule
%     \multicolumn{16}{c}{STGCN-NB Outputs} \\
%     \hline
%     {} & \multicolumn{7}{c}{Full observations} & \vline & \multicolumn{7}{c}{Sparsity-entry only} \\
%     \hline
%     Method & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
%     Interval    &  calibration    &  binning         &   regression       &   scaling   &    scaling &     &             &    \vline &  calibration        &      binning     &     regression     &          scaling  &    scaling    &   &         \\
%     \midrule
%     CCR\_1h       &        0.217 &     0.199 &    0.207 &    0.215  &  0.185 &  \underline{0.164}  &   \textbf{0.160} &       \vline & 0.524 &     0.189 &    \underline{0.129} &     0.500 &  0.362 &  0.269 & \textbf{0.001}     \\
%     CCR\_8h       &        0.315 &     0.097 &    \textbf{0.048} &     0.241 &  0.210 &    0.312   &\underline{0.109} &     \vline &   0.208 &     0.159 &    0.226 &     0.303 &  \underline{0.062} &  0.336 & \textbf{0.052}     \\
%     CCR\_1d    &        0.505 &     \underline{0.238} &    \textbf{0.185} &     0.468 &  0.873 & 0.330 &      0.275  &       \vline & 0.991 &     0.977 &    0.732 &     0.868 &  \textbf{0.208} &  0.330  & \underline{0.284}    \\
%     CCR\_1w       &        0.415 &     \underline{0.403} &     0.414&     0.416 &  1.965 & 0.260 & \textbf{0.342}      &     \vline &   0.145 &     1.084 &    0.143 &     \underline{0.105} &  0.151 &  0.108 & \textbf{0.058}    \\
    
%     \midrule
%     CTC\_1h       &        0.082 &     0.214 &    0.210 &       \underline{0.114}  &  0.163 &  0.048 &  \textbf{0.028} &      \vline &  0.042 &     0.702 &    0.579 &    0.381 &  0.596 & \underline{0.006} & \textbf{ 0.005}      \\
%     CTC\_8h       &        0.189 &     0.200 &    0.136 &       0.211 &  \underline{0.079} &  0.163  & \textbf{0.040}   &     \vline &   0.213 &     0.226 &    \underline{0.131} &     0.255 &  0.168 &  0.179 & \textbf{0.003}      \\
%     CTC\_1d    &        0.303 &     \underline{0.075} &    \textbf{0.060} &   0.422 & 0.265  &  0.170 &    0.079   &      \vline &  0.007 &     0.154 &    \underline{0.078} &     0.537 &  0.240 &  0.152 & \textbf{0.002}     \\
%     CTC\_1w       &        1.482 &     0.850 &    1.048 &     \underline{0.833} &  1.596 & 0.955 & \textbf{0.225}      &    \vline &    0.814 &     1.447 &    1.237 &     \underline{0.754} &  0.958 &  0.846 & \textbf{0.196}     \\

%     % \midrule
%     % SLD\_5min & & & & & & & & & & & & \\
%     % SLD\_15min & & & & & & & & & & & & \\
%     % SLD\_60min & & & & & & & & & & & & \\
%     \hline
%     \multicolumn{16}{c}{GWN-NB Outputs} \\
%     \hline
%     {} & \multicolumn{7}{c}{Full observations} & \vline & \multicolumn{7}{c}{Sparsity-entry only} \\
%     \hline
%     Method & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
%     Interval    &  calibration    &  binning         &   regression       &   scaling   &    scaling    &    &           &      \vline & calibration        &      binning     &     regression     &          scaling  &    scaling    &     &         \\
%     \midrule
%     CCR\_1h       &        0.904 &     0.796 &    0.838 &       1.978 &  0.769 &  \underline{0.220}   &\textbf{0.199} &       \vline &  0.377 &     0.451 &    0.658 &       0.378 &  0.322 &  \underline{0.211}  & \textbf{0.001} \\
%     CCR\_8h       &        2.585 &     0.640 &    0.618 &       1.257 &  \underline{0.415} &  0.483   &\textbf{0.378} &    \vline &    0.686 &     \underline{0.138} &    0.180 &       0.440 &  0.187 & 0.354    &\textbf{0.043} \\
%     CCR\_1d     &   1.186 &     0.883 &    1.024 &       3.270 &  1.006 &  \underline{0.427}   &\textbf{0.352}  &   \vline &     1.540 &     0.528 &    0.652 &       1.537 &  \underline{0.425} &  0.639   &\textbf{0.115} \\
%     CCR\_1w       &        2.990 &     0.384 &    \underline{0.307} &       2.503 &  \textbf{0.211} &  2.030  & 0.330 &    \vline &    3.736 &     0.387 &    \textbf{0.356} &       3.737 &  0.534 &  1.911  & \underline{0.308} \\
    
%     \midrule
%     CTC\_1h      & 0.381 & 0.355 & 0.341 & 0.334 &  0.434 & \underline{0.222} &\textbf{0.186} & \vline & 0.784 & 0.641 & 0.610 &       0.784 &  1.000 &  \underline{0.105} &\textbf{0.003} \\
%     CTC\_8h      & 0.931 & 0.416 &  0.388 & 1.381 &  \underline{0.169} & 0.226  &\textbf{0.148} &        \vline & 2.213 &     0.720 &    0.659 &       1.995 &  \underline{0.421} &  0.776   &\textbf{0.221}\\
%     CTC\_1d      & 0.523 & \underline{0.420} & 0.448 & 0.571 &  0.523 & 0.432   &\textbf{0.139}  &        \vline & 0.250 &     0.464 &    0.405 &       \underline{0.248} &  0.484 &   0.439  &\textbf{0.010} \\
%     CTC\_1w      & 0.408 & 0.114 & \underline{0.114} & 0.259 &  0.236 & 0.241 &\textbf{0.090} &        \vline & 0.466 &     0.479 &    \underline{0.436} &       0.457 &  0.451 &  0.476  &\textbf{ 0.350}\\
    
%     % \midrule
%     % SLD\_5min  & & & & & & & & & & & & \\
%     % SLD\_15min & & & & & & & & & & & & \\
%     % SLD\_60min & & & & & & & & & & & & \\
%     \bottomrule
%     \end{tabularx}
%     \caption{ENCE of the different calibration models. Bold fonts mark the best and underlines denote the second-best calibration models.}
%     \label{tab:ce_full}
% \end{table*}


\subsection{Data Description}
Two spatiotemporal datasets are used: (1) Chicago Traffic Crash Data (CTC) sourced from 277 police beats between January 1, 2016 and January 1, 2023; (2) Chicago Crime Records (CCR) derived from 77 census tracts spanning January 1, 2003 to January 1, 2023. Despite both CTC and CCR data originating from the Chicago area, their disparate reporting sources lead to different spatial units: census tracts for CCR and police beats for CTC. Both datasets use the first 60\% timesteps for training, 20\% for calibration and validation, and 20\% for testing.

The temporal resolutions of the datasets are varied to demonstrate the ubiquitous sparsity issue and its practical significance in spatiotemporal analysis. For example, four temporal resolutions are created for CTC and CCR datasets, with details available in Table \ref{tab:data_sparsity}. We designate the 1-hour and 8-hour cases of Crash and Crime datasets as sparse instances, due to a higher prevalence of zeros.

\begin{table}[ht]
    \centering
    \begin{tabular}{cc|cc}
    \toprule
        Dataset & Temporal resolution  & Size & Sparsity\\
    \midrule              
       \multirow{4}{*}{CCR}  & \cellcolor{Gray}1-hour & \cellcolor{Gray}(77, 175321)& \cellcolor{Gray}67\%\\
       & \cellcolor{Gray}8-hour & \cellcolor{Gray}(77, 21916) & \cellcolor{Gray}18\%\\
       & 1-day  & (77, 7306)  & 4\%\\ 
       & 1-week & (77, 1044)& $<0.1\%$\\
    \midrule
       \multirow{4}{*}{CTC}  & \cellcolor{Gray}1-hour & \cellcolor{Gray}(277, 61369) & \cellcolor{Gray}96\% \\   
       & \cellcolor{Gray}8-hour & \cellcolor{Gray}(277, 7672) & \cellcolor{Gray}76\% \\
       & 1-day  & (277, 2558) & 47\% \\
       & 1-week & (277, 366) & 7\% \\
    % \midrule        
    %       \multirow{3}{*}{SLD}  & \cellcolor{Gray}5min  &  \cellcolor{Gray}(4489, 34560) & \cellcolor{Gray}88\% \\
    %       & 15min &  (4489, 11520) & 70\% \\
    %       & 60min &  (4489, 2880)  & 50\% \\          
    \bottomrule
    \end{tabular}
    \caption{Characteristics of various datasets showing variation in sparsity at different temporal resolutions. Dataset sizes are represented as (spatial, temporal) dimension pairs. Sparse cases are marked grey.}
    \label{tab:data_sparsity}
\end{table}

For adjacency matrices, we calculate geographical distances $d_{ij}$ between centroids of regions $i$ and $j$, be they census tracts or police beats. This distance is then transformed into a similarity measure, $\mathbf{A}_{ij} = e^{-d_{ij}/0.1}$, where $0.1$ is a scaling parameter, thus forming an adjacency matrix.

\subsection{Modified Spatiotemporal Models}
In order to demonstrate our model's ability to generalize on spatiotemporal prediction models, we modify two existing popular spatiotemporal forecasting models: Spatio-temporal Graph Convolution Network (STGCN) \citep{yu2017spatio}, Graph WaveNet (GWN) \citep{wu2019graph}, and \redfont{DSTAGNN}. They are designed for numerical value outputs. We modify their last layer from single numerical output to the location parameter $\mu$ and the dispersion parameter $\alpha$ of negative binomial distributions. Two linear layers are added in the tail of the neural network structures to learn the parameters. We renamed the modified model as STGCN-NB and GWN-NB respectively. Besides, we modify the loss function from mean square error loss to the likelihood loss defined in Equation \ref{eq:modify_loss}:
\begin{equation}
\begin{aligned}
& \mathcal{L}(\mu, \alpha, y) = -\left[y \cdot \log\left(\frac{\mu + \epsilon}{\mu + \alpha + 2\epsilon}\right)\right] \\
&\quad\quad - \Gamma(y + \alpha + \epsilon) + \Gamma(y + 1) + \Gamma(\alpha + \epsilon) \\
&\quad\quad - \alpha \cdot \log\left(\frac{\alpha + \epsilon}{\mu + \alpha + 2\epsilon}\right) + \lambda \cdot ||\alpha||^2
\label{eq:modify_loss}
\end{aligned},
\end{equation}
where $y$ is the target variable, $\mu$ and $\alpha$ are model outputs, $\Gamma$ is the gamma function, $\lambda$ is the regularization parameter, and $\epsilon$ is a small constant added to improve numerical stability. Equation \ref{eq:modify_loss} is derived from the NB likelihood controlled by $\mu$ and $\alpha$.

\begin{table}[ht]
    \centering
    \begin{tabular}{ccc}
    \toprule
        Dataset & STGCN & GWN \\
    \midrule              
        CCR\_1h & 0.637 (0.703) & 0.962 (0.766) \\
        CCR\_8h & 2.386 (2.326) & 2.052 (2.376) \\
        CTC\_1h & 0.214 (0.220) & 0.980 (0.220) \\
        CTC\_8h & 0.633 (0.726) & 0.924 (0.746) \\
    \bottomrule
    \end{tabular}
    \caption{RMSE of original model outputs and the modified models (shown in the parenthesis) using sparse datasets.}
    \label{tab:model_modification}
\end{table}

The loss function ensures the predicted Negative Binomial distribution aligns well with the true target values. It penalizes predictions where the mean of the distribution ($\mu$) is far from the actual target values. Furthermore, it incorporates the shape of the distribution via the dispersion parameter ($\alpha$) to capture the variability in the data. The loss function also includes a regularization term to prevent overfitting by discouraging overly large values of $\alpha$.



As shown in Table \ref{tab:model_modification}, the model modification is successful without a loss of accuracy. In fact, the NB modification shows better performance in the sparse dataset as the NB distributions are more suitable for the nature of discrete data. 

% Detailed numerical comparisons can be found in \redfont{Appendix}.




% excluding calibration techniques that incorporate uncertainty during training \citep{thiagarajan2020building,huang_uncertainty_2023}
\begin{table*}[!h]
    \scriptsize
    \centering    
    \begin{tabularx}{\linewidth}{c*{7}{>{\centering\arraybackslash}X}@{\hspace{4pt}}c@{\hspace{4pt}}*{7}{>{\centering\arraybackslash}X}}
    \toprule
    \multicolumn{16}{c}{\textbf{STGCN-NB Outputs}} \\
    \hline
    {} & \multicolumn{7}{c}{Full observations} & \vline & \multicolumn{7}{c}{Zero-only targets} \\
    \hline
    Method / & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
    Interval    &  calibration    &  binning         &   regression       &   scaling   &    scaling &     &             &    \vline &  calibration        &      binning     &     regression     &          scaling  &    scaling    &   &         \\
    \midrule
    CCR\_1h       &     1.160 &     0.410 &    0.517 &    0.887     &  0.443  &   \underline{0.235}  & \textbf{0.198}  &    \vline  &   1.167 &     0.361 &  0.386   &   0.473   &  0.477 &  \underline{0.273} &  \textbf{0.267}  \\
    CCR\_8h       &   1.389 &   \underline{0.344}   &    0.417 &    0.385  &  0.373 &  0.392 &  \textbf{0.336}    &  \vline  &   1.065 &     0.568 &    0.578 &       0.427 &  \underline{0.162} &  0.175  & \textbf{0.127}  \\
    CCR\_1d       &    0.413 &     0.593 &    0.546 &       0.364 &  \underline{0.294} &  0.297  &  \textbf{0.192}   &  \vline  &  1.266 &     1.047 &    0.979 &       1.167 &  \underline{0.840}  &    0.843    &  \textbf{0.738} \\
    CCR\_1w       &   0.855 &     0.784 &    0.773 &       0.765 &  0.579 & \underline{0.272} &    \textbf{0.242}   &    \vline  &   0.354 &     0.362 &    0.332 &       0.287 &  0.345 &  \underline{0.155}  &  \textbf{0.113}  \\    
    \midrule
    CTC\_1h       &    0.578 &     0.227 &    \underline{0.200} &       1.390 &  0.452 &  0.388 &   \textbf{0.165}  &       \vline  &   3.211 &     0.415 &    \underline{0.363} &       2.042 & 0.646 &  0.416  &   \textbf{0.078} \\
    CTC\_8h       &   0.323 &     0.320 &    0.255 &       0.570 &  0.297 &  \underline{0.241}  &  \textbf{0.233}   &       \vline  &  0.330 &     0.247 &    0.276 &       0.551 &  0.230 &  \underline{0.196}  &  \textbf{0.184} \\
    CTC\_1d       &   0.722 &     0.050 &     \textbf{0.011}  &       0.862 &  0.060 &  0.048  &  \underline{0.047} &       \vline  &  0.434 &     0.128 &    \textbf{0.027} &       5.451 &  0.152 &  0.379  & \underline{0.150}  \\
    CTC\_1w       &     2.279 &     1.227 &    1.527 &       0.914 &  2.265 &  \underline{0.378}   & \textbf{0.365} &       \vline  &  1.823 &     2.384 &    2.009 &       1.160 &  1.343 &  \underline{0.767}  &  \textbf{0.755}  \\

    % \midrule
    % SLD\_5min & & & & & & & & & & & & \\
    % SLD\_15min & & & & & & & & & & & & \\
    % SLD\_60min & & & & & & & & & & & & \\
    \hline
    \hline
    \multicolumn{16}{c}{\textbf{GWN-NB Outputs}} \\
    \hline
    {} & \multicolumn{7}{c}{Full observations} & \vline & \multicolumn{7}{c}{Zero-only targets} \\
    \hline
    Method / & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC & \vline & Before & Histogram & Isotonic & Temperature &  Platt & QR & SAUC \\
    Interval    &  calibration    &  binning         &   regression       &   scaling   &    scaling    &    &           &      \vline & calibration        &      binning     &     regression     &          scaling  &    scaling    &     &         \\
    \midrule
    CCR\_1h       &  1.200 &     1.022 &   0.889   &   1.149   &  0.834 & \underline{0.604}  & \textbf{0.493}   &   \vline  &  2.042 &     1.796 &    1.274 &       1.710 &  1.356 &  \underline{0.476}  &  \textbf{0.375} \\
    CCR\_8h       &    0.670 &     0.636 &    0.612 &   0.696 &  0.655 &  \underline{0.597} & \textbf{0.566}   &       \vline  &  1.398 &     0.389 &    0.492 &    1.179    &  0.478 &  \underline{0.308}   &  \textbf{0.186}   \\
    CCR\_1d       &   0.997  &     0.662 &    0.633 &    0.581 &  \underline{0.562} & 0.587  &  \textbf{0.504} &       \vline  &  1.158 &     0.583 &    \underline{0.580} &       0.725 &  0.747 &  0.644  & \textbf{0.563}  \\
    CCR\_1w       &    0.858 &     0.938 &    0.935 &       \textbf{0.611} &  0.931 &  0.857 &  \underline{0.829}  &       \vline  &  0.335 &     0.218 &    0.219 &       \textbf{0.161} &  0.219 & 0.250  &  \underline{0.172}    \\
    
    \midrule
    CTC\_1h      &   0.868  &  0.816  &  0.891  &  0.859  & \underline{0.634}  &  0.832  &  \textbf{0.290}  &  \vline  & 1.300  &  0.712  &  0.561  & 1.001  &  \underline{0.143}  &  0.998  & \textbf{0.139}  \\
    CTC\_8h      & 0.931 & 0.416 &  0.388 & 1.381 &  \underline{0.169} & 0.226  &\textbf{0.148} &        \vline & 2.213 &     0.720 &    0.659 &       1.995 &  \underline{0.421} &  0.776   &\textbf{0.221}\\
    CTC\_1d      & 0.523 & \underline{0.420} & 0.448 & 0.571 &  0.523 & 0.432   &\textbf{0.139}  &        \vline & 0.250 &     0.464 &    0.405 &       \underline{0.248} &  0.484 &   0.439  &\textbf{0.210} \\
    CTC\_1w      & 0.408 & 0.115 & \textbf{0.114} & 0.259 &  \underline{0.236} & 0.241 &0.239 &        \vline & 0.466 &     0.479 &    \textbf{0.436} &       0.457 &  0.451 &  0.476  & \underline{0.450}\\
    
    % \midrule
    % SLD\_5min  & & & & & & & & & & & & \\
    % SLD\_15min & & & & & & & & & & & & \\
    % SLD\_60min & & & & & & & & & & & & \\
    \bottomrule
    \end{tabularx}
    \caption{ENCE of the calibration models. Bold fonts mark the best and underlines denote the second-best calibration results.}
    \label{tab:ce_full}
\end{table*}

\subsection{Baseline Calibration Methods}
The SAUC will be compared to the baseline post-hoc calibration methods proven to be effective in the regression tasks using cross-sectional data. The baseline methods include:
\begin{itemize}
    \item \noindent\textit{Isotonic regression} \citep{niculescu2005predicting}, a non-parametric technique, which ensures non-decreasing predictive probabilities, assuming higher model accuracy with increased predicted probabilities;

    \item \noindent\textit{Temperature scaling} \citep{kull2019beyond}, which scales the model's output using a learned parameter, whose efficacy for regression models depends on the output's monotonicity in relation to confidence;

    \item \noindent\textit{Histogram binning} \citep{zadrozny2001obtaining}, a method partitioning predicted values into bins, calibrating each independently according to observed frequencies, yet might lack flexibility for diverse prediction intervals;

    \item \noindent\textit{Platt Scaling} \citep{kuleshov2018accurate}, which applies a scaling transformation to the predicted values with the function derived from minimizing observed and predicted value discrepancies, providing linear adaptability but potentially inadequate for complex uncertainty patterns;
    \item \noindent\textit{Quantile regression} \citep{chung2021beyond}, aforementioned.
\end{itemize}


% \noindent\textit{Quantile regression} \citep{chung2021beyond}, an approach that minimizes the absolute difference between observed and predicted values using an asymmetrically weighted objective function, rendering it appropriate for calibration of asymmetric distributions.




% \begin{figure*}[!t]
%     \centering    
%     \subfigure[Calibration result using full data]{\includegraphics[scale=0.95]{figs/calibration_crime_1h.pdf}\label{fig:ccr1h_full}}
%     \subfigure[Calibration result using sparsity entries only]{\includegraphics[scale=0.95]{figs/calibration_crime_zero_1h.pdf}\label{fig:ccr1h_zero}}
%     \caption{Different calibration methods comparison on different components of STGCN-NB model outputs on data CCR\_1h.}
%     \label{fig:ccr1h}
% \end{figure*}



% \vspace{-5pt}
\subsection{Calibration Results Comparison}

% In our study, we applied an array of calibration methodologies to models trained using 60\% of the dataset. These models output parameters $\mu$ and $\alpha$, which in turn yield mean value predictions and PIs. We then recalibrated these models using an independent validation set, adjusting parameters for techniques such as temperature scaling, isotonic regression, Platt scaling, and quantile regression. A novel facet of our approach was the introduction of sparsity-aware calibration, where predictions with mean values below $0.5$ were identified as zero. This approach allowed for the calibration of models tailored specifically for this subset of data. For computing ENCE on ground-truth zero values, we used genuinely zero data instances, thereby ensuring precise uncertainty calibration measurement.

The calibration performance of the initial models and our proposed calibration methods is presented in Table \ref{tab:ce_full}, assessed via ENCE on two adapted spatiotemporal prediction models. The ``zero-only targets'' refers to computing the ENCE exclusively on the true target values that are zeroes.

Table \ref{tab:ce_full} denotes superior performance within each dataset with bold type and underlines the second-best results. Our findings reveal that the SAUC method typically outperforms other models, though it might fall short in aggregated cases, such as those with a 1-week resolution. Interestingly, the SAUC method achieved approximately a 23\% reduction in ENCE compared to the second-best model when using full observations and also about a 20\% reduction in sparsity entries. The separation of zero and non-zero data during calibration proved particularly beneficial, effectively addressing the issues of heteroscedasticity and zero inflation, commonly found in real-world datasets. However, we observed that calibration methods sometimes do not improve, or even worsen, calibration errors, mainly due to overfitting on the calibration set, a problem particularly evident in temperature scaling and isotonic regression methods. 

On a general note, histogram binning and isotonic regression showed similar calibration results among baseline models as Equation \ref{eq:cdf} is non-decreasing, which makes the two methods easier to fit. Temperature scaling provides better calibration results in coarse temporal resolution scenarios and Platt scaling excels in sparse cases. QR consistently ranks as the second-best model in many cases, and our SAUC method has a close performance as QR in aggregated non-sparse cases but excels notably in sparse cases.


\subsection{Reliability Diagram Evaluation}

Utilizing Equations~\ref{eq:define_calib} and~\ref{eq:ence}, we refine the conventional reliability diagram to evaluate the calibration efficacy of a model \citep{kull2019beyond}. This involves partitioning predictions into bins based on $\mathcal{I}$, after which we compute the RMSE and MPIW employing the calibrated $\mu^*$ and $|\mathcal{I}^*|$ for each respective bin.

Figure \ref{fig:ccr8h} presents a comparative reliability diagram of STGCN-NB outputs prior to calibration, alongside Isotonic regression, Platt scaling, and our SAUC technique, each applied to different segments of the CCR\_8h dataset. We selectively feature representative non-parametric and parametric baseline calibration approaches based on their performance. The diagonal dashed line symbolizes the calibration ideal: a closer alignment to this line indicates superior calibration.

\begin{figure*}[!ht]
    \centering    
    \subfigure[Full observations, CCR\_8h]{\includegraphics[scale=1]{figs/calibration_crime.pdf}\label{fig:ccr8h_full}}
    \subfigure[Zero-only targets, CCR\_8h]{\includegraphics[scale=1]{figs/calibration_crime_zero.pdf}\label{fig:ccr8h_zero}}
    \subfigure[Full observations, CCR\_1h]{\includegraphics[scale=1]{figs/calibration_crime_1h.pdf}\label{fig:ccr1h_full}}
    \subfigure[Zero-only targets, CCR\_1h]{\includegraphics[scale=1]{figs/calibration_crime_zero_1h.pdf}\label{fig:ccr1h_zero}}    
    \caption{Reliability diagrams of different calibration methods applied to STGCN-NB outputs on different components of CCR\_8h and CCR\_1h data. Results closer to the diagonal dashed line are considered better.}
    \label{fig:ccr8h}
\end{figure*}

A closer examination of Figure \ref{fig:ccr8h_full} reveals that both baseline models and our SAUC technique adeptly calibrate the model outputs across all observations. Yet, focusing solely on the reliability diagram of our calibrated outputs for ground-truth zero values, as depicted in Figure \ref{fig:ccr8h_zero}, there is a noticeable deviation from the ideal line. Conversely, our SAUC approach demonstrates commendable alignment with the ideal when authentic data are zeros. This observation remains consistent for the CCR\_1h dataset, as seen in Figures \ref{fig:ccr1h_full} and \ref{fig:ccr1h_zero}. By juxtaposing Figures \ref{fig:ccr8h_full} and \ref{fig:ccr1h_full}, it becomes evident that the calibration performance diminishes in scenarios with finer resolutions. Nevertheless, our SAUC technique retains commendable efficacy, particularly when predicting zero entries, attributed to our distinctive calibration approach coupled with QR's adeptness at managing heteroscedasticity, especially when predictions on zeros exhibit considerable variability. Contemporary probabilistic spatiotemporal prediction models predominantly prioritize refining MPIWs for enhanced accuracy, often unintentionally neglecting practical safety considerations. Our calibration strategy offers outputs with reinforced reliability.

\subsection{Spatial Evaluation}
To evaluate the use of SAUC outputs, we introduce Risk Score (RS), an enhancement of the traditional metric defined as the product of \textit{event probability} and \textit{potential loss magnitude} \citep{ng2002algorithm,vose2008risk}:

\begin{equation}
RS = \hat{\mu} \times |\hat{\mathcal{I}}|.
\end{equation}

This metric integrates anticipated risk ($\hat{\mu}$) and prediction uncertainty ($|\hat{\mathcal{I}}|$), attributing higher RS to regions with both high incident frequency and uncertainty. This RS metric assigns higher risk to predictions that are characterized by both large predicted mean values and high uncertainty.


\begin{figure}[!ht]
    \centering
    \subfigure[Avg. number of crashes]{\includegraphics[width=0.23\textwidth]{figs/case_study_expected.pdf}\label{fig:case_study_expect}}   \hfill 
    \subfigure[RS distribution using prediction before calibration]{\includegraphics[width=0.23\textwidth]{figs/RS_before_avg.pdf}\label{fig:case_study_before}}
    
    \subfigure[RS distribution using calibrated prediction via Platt scaling]{\includegraphics[width=0.23\textwidth]{figs/RS_calib_baseline.pdf}\label{fig:case_study_baseline}} \hfill
    \subfigure[RS distribution using using calibrated prediction via SAUC]{\includegraphics[width=0.23\textwidth]{figs/RS_calib_avg.pdf}\label{fig:case_study_calib}}
    \caption{Traffic crash accident distributions and calibration using CTC\_8h data. All the data are averaged over the temporal dimension.}
    \label{fig:case_study}
\end{figure}

Using the CTC\_8h dataset, we demonstrate the importance of SAUC for evaluating the risks of traffic accidents. Figure \ref{fig:case_study} juxtaposes the average number of crashes and average RS values over time for each region, pre and post-calibration. Prior to calibration, as depicted in Figure \ref{fig:case_study_before}, the RS in regions, especially Chicago's northern and southern sectors, did not provide actionable insights, given their frequent traffic incidents reported by Figure \ref{fig:case_study_expect}. This is due to the tight PIs from pre-calibration model outputs lower the RS. As shown in Figure \ref{fig:case_study_baseline}, RS distribution from Platt scaling calibrated predictions could highlight certain risky areas, but still miss the major crash regions in southern Chicago. In contrast, SAUC-derived predictions, as seen in Figure \ref{fig:case_study_calib}, unveil coherent spatial distribution patterns highly consistent with Figure \ref{fig:case_study_expect}, demonstrating the effectiveness for urban safety monitoring.

Rather than just yielding exact numerical predictions with tight confidence intervals, it is imperative that models convey equivalent severity levels when integrating uncertainty. Such an approach ensures reliable outputs in crime and accident predictions. Notably, the variance between zero and one incident counts is pivotal in risk management. Existing probabilistic prediction studies focus on exact values and restricted confidence bounds, sometimes neglecting the variability, especially around zero incidences.

% \footnote{\url{https://rshah.carto.com/viz/8683f768-3188-11e4-94b1-0e230854a1cb/public_map}}.

\subsection{Deployment}

Also add more recent GNN models

\redfont{Add ablation study to say the Gaussian distribution is worse.}

==> backup_sections/6.Conclusion.tex <==
\section{Conclusion}
Existing spatiotemporal GNN models primarily predict deterministic values, which neglect the uncertainties inherent in data. Particularly the high-resolution spatiotemporal data is largely sparse and exhibits asymmetric distributions, so it presents further challenges to quantify the uncertainty. To address this challenge, in this paper, we propose the SAUC method that calibrates uncertainties across both zero and non-zero values. By transforming GNN-based deterministic models to probabilistic ones, SAUC aligns predictions with the zero-inflated nature of spatiotemporal datasets. We also design novel PI-based calibration metrics for sparse and asymmetric distributions. Empirical assessments on two real-world datasets demonstrate the efficacy of the SAUC method, with a 20\% reduction in calibration errors for zero-only targets in sparse cases. SAUC not only complements existing GNN models but also can be used for risk evaluation in sparse datasets where reliable predictions are imperative due to inherent safety concerns.

\section{Ackowledgement}
This material is based upon work supported by the U.S. Department of Energy’s Office of Energy Efficiency and Renewable Energy (EERE) under the Vehicle Technology Program Award Number DE-EE0009211.

==> backup_sections/kdd_2024_rebuttal.tex <==
\newpage
\section{Contents based on the rebuttals}
\subsection{Why the proposed calibration metric ENCE is preferred?}
For each future point, we will predict a mean value and the confidence interval. N data future data points will have N different confidence intervals. Therefore, variability is not measurable for each CI because there is only one predicted value for this CI.

That’s why we need mean prediction interval width of the N data points (we further divide them into bins and calculate the MPIW within each bins) instead of simply using the CI as the variability. It is not measurable for single predicted points, but a bin of data pints. Following this idea, we replace the data variability with some error terms, like RMSE and quantify the uncertainty using MPIW, leading to the usage of exiting metric.

We have also included the experiments using coverage of CI as the metrics before and after calibration. We show the comparison of coverage of quantiles before and after the calibration. The coverage is calculated as how many points fall within the confidence interval, following the same notation schema from the manuscript, it is written as:

\begin{equation}
\text{Coverage}_{0.05-0.95} = \frac{1}{|U|} \sum_{i \in U} 1_{(y_i \geq \hat{F}_i^{-1}(0.05) \, \& \, y_i \leq \hat{F}_i^{-1}(0.95))} \approx 0.9
\end{equation}

where $\hat{F}_i^{-1}(0.05)$ and $\hat{F}_i^{-1}(0.95)$ are the predicted confidence intervals, which are obtained from the model output or the calibrated model output. We expect the portion of true data from the test set that falls within the 5\%-95\% confidence interval should be approximately 0.9.

To have the monotonic comparison, we use the metric:

\begin{equation}
C^* = |0.9 - \text{Coverage}_{0.05-0.95}|
\end{equation}

to measure the closeness between the predicted confidence intervals and the expected 90\% data coverage. This is the absolute value of the subtraction of 0.9 from the coverage of the predicted distribution. Smaller values are better, i.e., the ideal case is 0.

We compare the metric $C^*$ using the confidence interval outputted by STGCN-NB before and after our calibration methods.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Before Calibration} & \textbf{After Calibration} \\
\hline
CCR\_1h & 0.311 & 0.099 \\
CCR\_8h & 0.347 & 0.040 \\
CCR\_1d & 0.364 & 0.056 \\
CCR\_1w & 0.457 & 0.041 \\
CTC\_1h & 0.311 & 0.122 \\
CTC\_8h & 0.313 & 0.128 \\
CTC\_1d & 0.316 & 0.129 \\
CTC\_1w & 0.463 & 0.140 \\
\hline
\end{tabular}
\caption{Comparison of $C^*$ before and after calibration}
\end{table}

Generally speaking, the calibrated confidence interval can better cover the data variability, as demonstrated by the significant decrease in the metric $C^*$.

\subsection{Comparing NB and Poisson Distribution}
Is the NB distribution flexible enough to capture the response distributions? We have implemented Poisson distribution as our model's estimated distribution. 

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Original STGCN} & \textbf{STGCN-NB} & \textbf{STGCN-Poisson} \\
\hline
CCR\_1h & 0.637 & 0.703 & 0.581 \\
CCR\_8h & 2.386 & 2.326 & 2.419 \\
CTC\_1h & 0.214 & 0.220 & 0.282 \\
CTC\_8h & 0.633 & 0.726 & 0.962 \\
\hline
\end{tabular}
\caption{RMSE comparison of original model, NB modification, and Poisson modification.}
\end{table}

It is clear that the Poisson modification has similar performance to the NB distribution based on the experiment results. The NB distribution is slightly better. The experiment shows that NB could be a potentially flexible distribution to capture the uncertainty.

\subsection{Related work about probabilistic/Bayesian models}
\redfont{Add some more Bayesian model citations}

Thanks for pointing this out! In Section 2.1 We have demonstrated that the frequentist (predicting the confidence interval or variance directly) and Bayesian models are the two mainstreamed uncertainty quantification approaches, and we mainly focus on the frequentist approach as it is widely discussed in the deep learning communities.

Bayesian models could potentially be another aspect of solving the problem. However, it requires the assumptions of models from the start and it will be a bit difficult to generalize to existing neural networks, as we need to ensure to follow the holistic process of the Bayesian approach.

We have reviewed the references and will include them in the later version of the manuscript.

\subsection{Sensitivity analysis}
\subsubsection{Sensitivity Analysis of Number of Bins}

We choose the bin number from the range \texttt{bin\_nums = [1, 5, 10, 15, 20, 25, 30]} and discuss the ENCE change with respect to the bin number. Note that we fix the threshold to 0.5 when performing the uncertainty calibration. We conduct the sensitivity analysis using the four cases in the crime dataset using STGCN-NB model outputs.

\begin{table}[h!]
\centering
\caption{ENCE on the full observations with respect to different bin numbers.}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset/Bin} & \textbf{1} & \textbf{5} & \textbf{10} & \textbf{15} & \textbf{20} & \textbf{25} \\
\hline
CCR\_1h & 0.513 & 0.302 & 0.299 & 0.198 & 0.249 & 0.292 \\
CCR\_8h & 0.096 & 0.113 & 0.185 & 0.336 & 0.123 & 0.115 \\
CCR\_1d & 0.093 & 0.167 & 0.185 & 0.192 & 0.189 & 0.207 \\
CCR\_1w & 0.074 & 0.216 & 0.323 & 0.242 & 0.254 & 0.272 \\
\hline
\end{tabular}
\end{table}

\begin{table}[h!]
\centering
\caption{ENCE on the zero-only observations with respect to different bin numbers.}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset/Bin} & \textbf{1} & \textbf{5} & \textbf{10} & \textbf{15} & \textbf{20} & \textbf{25} \\
\hline
CCR\_1h & 0.650 & 0.689 & 0.604 & 0.267 & 0.229 & 0.501 \\
CCR\_8h & 0.642 & 0.583 & 0.504 & 0.127 & 0.172 & 0.345 \\
CCR\_1d & 0.641 & 1.181 & 1.096 & 0.738 & 1.025 & 0.958 \\
CCR\_1w & 1.445 & 0.950 & 0.361 & 0.113 & 0.363 & 0.567 \\
\hline
\end{tabular}
\end{table}

\subsubsection{Sensitivity Discussion}
From Tables 1 and 2, we can see that the number of bins impacts the ENCE. Both smaller bin sizes and larger bin numbers may not yield good ENCE in the end.

This is intuitive to understand. For example, if there is only one bin, all the data points fall within the same bin, thus we compare the average data variability with the average MPIW using all the data. It is hard to differentiate different levels of variance. On the other hand, if only a few data points lie within a bin, the results will also fluctuate due to the small sample size. Therefore, a bin number between 10 and 20 is preferable.

\subsubsection{Runtime Discussion}
The complexity of the algorithm proportionally depends on the size of the data. From the runtime table, you can see that by reducing the resolution from 1 hour to 8 hours, 1 day, and 1 week, the runtime drops nearly proportionally to the resolution change.

\subsection{Complexity discussion}
Since our method is a post-hoc method, the added complexity is easier to address in terms of runtime. Based on the same experiment settings as the sensitivity analysis, the runtime discussion is shown in Figure \ref{tab:runtime}.

\begin{table}[h!]
\centering
\caption{Run time of the calibration models on the full observations with respect to different bin numbers.}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset/Bin} & \textbf{1} & \textbf{5} & \textbf{10} & \textbf{15} & \textbf{20} & \textbf{25} \\
\hline
CCR\_1h & 19m52s & 22m10s & 19m41s & 20m52s & 18m42s & 18m04s \\
CCR\_8h & 6m24s & 5m33s & 5m33s & 5m33s & 5m32s & 5m07s \\
CCR\_1d & 2m29s & 1m54s & 1m49s & 1m40s & 1m50s & 1m33s \\
CCR\_1w & 30s & 13s & 14s & 12s & 14s & 10s \\
\hline
\end{tabular}
\label{tab:runtime}
\end{table}
The complexity of the algorithm proportionally depends on the size of the data. From the runtime table, you could see that by reducing the resolution from 1hour to 8 hours, 1day, and 1 week, the runtime drops nearly proportionally to the resolution change.

\subsection{How are the methods applied for non-Spatiotemporal data?}
This will be an interesting topic to extend in the future. So far, our calibration methodology is based on the spatiotemporal GNN models, but our derivation is free from the spatiotemporal characteristics, for example, the spatial continuity and temporal effects, which means our calibration methods could be extended to non-spatiotemporal cases. Currently, our main applied datasets are still sparse spatiotemporal which is the main employed dataset, and it will be deviated from our main focus in this paper. We will consider extending it to a more general case and test on the non-spatiotemporal dataset in the future.


